New directions in the applications of rough path theory

This article provides a concise overview of some of the recent advances in the application of rough path theory to machine learning. Controlled differential equations (CDEs) are discussed as the key mathematical model to describe the interaction of a stream with a physical control system. A collection of iterated integrals known as the signature naturally arises in the description of the response produced by such interactions. The signature comes equipped with a variety of powerful properties rendering it an ideal feature map for streamed data. We summarise recent advances in the symbiosis between deep learning and CDEs, studying the link with RNNs and culminating with the Neural CDE model. We concluded with a discussion on signature kernel methods.

==> Signatures IEEE/other/math_commands.tex <==
% Definitions
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% \DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

% \mathbf -> \mb (math bold, bold math results in different letters)
\newcommand{\mb}[1]{\mathbf{#1}}

% \mathrm -> \mrm
\newcommand{\mrm}[1]{\mathrm{#1}}

% Nice fractions
\newcommand{\ttfrac}[2]{\nicefrac{#1}{#2}}

% Math letters
\def\reals{{\mathbb{R}}}
\def\seqs{{\mathcal{S}}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\len}{\mathrm{Length}}
\def\to{{\rightarrow}}
\def\dd{\mathrm{d}}
\def\bx{\mathbf{x}}
\def\bX{\mathbf{X}}
\newcommand{\Xx}{\bX_{t}}
\def\logsig{\mathrm{LogSig}}
\def\sig{\mathrm{Sig}}

% 
\newcommand{\ith}[1]{$#1^{\mrm{th}}$}

==> Signatures IEEE/other/ncdes_old.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/node_vs_ncde.png}
%     \caption{Visual comparison on the RNN, ODE-RNN and Neural CDE methods. \textbf{Left:} the RNN updates the hidden state only at observation times and is undefined in-between. \textbf{Middle:} The ODE-RNN is defined between observations and modifies the hidden state at each observation. \textbf{Right:} The Neural CDE model first constructs a continuous time path control $\Xx$ resulting in a true continuous time interpretation of the hidden state.}
%     \label{fig:rnn_odernn_ncde}
% \end{figure*}

\subsection{Neural ODEs}
Neural ODEs seek to predict some output $y \in \reals^q$ from data $x \in \reals^d$ by learning a function $f_\theta \colon \reals^v \rightarrow \reals^v$ and linear maps $\ell^1_\theta \colon \reals^d \rightarrow \reals^v, \ell^2_\theta \colon \reals^v \rightarrow \reals^w$ such that 
\begin{multline}
    y \approx \ell^2_\theta(z_n) \;\; \text{where} \;\; z_{t} = z_{t_0} + \int^t_{t_0} f_\theta(z) \dd t \\ \text{and} \;\; z_0 = \ell^1_\theta(x).
    \label{eq:node}
\end{multline}
Neural ODEs provide us with an interface between the fields of machine learning and differential equation modelling. They allow us to combine modern tools from ODE research alongside the high flexibility and powerful function approximation properties from machine learning.

However, the definition as stated in \Cref{eq:node} cannot be straightforwardly applied to stream data. The key issue is that a Neural ODE defines an initial value problem; once $\theta$ has been learnt, the solution to \Cref{eq:node} is determined by the initial condition at $z_0$ with no direct mechanism for incorporating data that arrives later. 

To get around this issue, we must encode all information into the hidden state $z_0$ prior to running the Neural ODE model. This is an unnatural way to process sequential data and motivates the question of whether there is an extension that can process stream-like data, such as a time series.

\subsection{Neural CDEs}
The aforementioned issues with Neural ODEs can be naturally addressed by modelling the data with a CDE. After all, CDEs and rough path theory are really the study of how to incorporate (potentially complex and highly oscillatory) incoming signals to update some state. \james{Terry can you improve this sentence.}

Start by supposing we observe some discrete time series $\bx = \big((t_0, x_0), \ldots, (t_n, x_n) \big)$ with $t_i \in \reals$ denoting the timestamp of the observation vector $x_i \in (\reals \cup \{*\})^{d-1}$, where $*$ is used to denote that some information may be missing, and $t_0 < \ldots < t_n$. 

The first problem we have is that we (in general) observe a discrete data process but CDE theory relies on continuous time signals. Therefore, the first thing we must do is create a continuous time embedding of the discrete data process. Let $\Xx \colon [0, n] \rightarrow \reals^d$ be some interpolation of the data such that $\Xx(i) = (t_i, x_i)$, where `$=$' denotes equality up to missing data. We use the subscript $_\bx$ to highlight the dependence on the underlying discrete data process. The path $\Xx$ is often referred to as the \textit{control}. 

%% something about missing data
Our allowances for missing data may seem a little odd notationally, but keeping open the possibility for missing data is important. Often when observing real-world data we do not see all features simultaneously; for example, when patient laboratory tests are returned in an ICU we only see those that were requested by the doctor, with other information being missing. Our definition is also broad enough that it allows for the possibility of data that is irregularly sampled, another common property of real-world time series data. 

Issues of missingness and sampling irregularity are pervasive in real-world data and have historically posed a challenge when it comes to developing modelling frameworks. Recurrent neural networks (RNNs) have been the dominant modelling class for complex time series data across a range of domains \citep{sutskever2011generating,mikolov2010recurrent,graves2014towards}; however, they require regularly sampled and fully observed data, with standard workarounds being to divide the interval into equally-sized bins, and impute missing observations using averages. Such methods necessarily result in a loss of information.

%% something about how Neural Cdes fixes this problem

This time we take $f_\theta \colon \reals^v \rightarrow \reals^{v \times d}$. We then say the solution $z \in \reals^v$ to
\begin{equation}
    z_t = f_\theta(z_t) \dd \Xx \quad z_{t_0} = \zeta,
    \label{eq:ncde}
\end{equation}
is the solution of a \textit{neural controlled differential equation}. Here ``$f_\theta(z_s) \dd \Xx$'' denotes a matrix-vector product.

This can be written in the equivalent integral form
\begin{equation}
    \quad z_{t} = z_{t_0} + \int^t_{t_0} f_\theta(z_s) \dd \Xx.
    \label{eq:ncde_integral}
\end{equation}
from which the comparison to the Neural ODE from \cref{eq:node} becomes clear. We have simply replaced $\dd t \rightarrow \dd \Xx$. This seemingly minor modification is what enables our Neural CDE model to change continuously based on incoming data, since the path $\Xx$ adapts the dynamics of the system via the $\dd \Xx$ term. 

\subsection{The rough update}
Before proceeding, we must first understand how to evaluate the Neural CDE equation from \Cref{eq:ncde}. Whilst the modification of $\dd t \rightarrow \dd \Xx$ may seem a simple one, we are left now with a path integral for which the method of solution is not immediately clear.

Thankfully, the solution to this problem has already been addressed in the field of rough paths in the form of a method known as -- \textit{the log-ODE method} -- that can approximate the solution of any CDE equation to a corresponding ODE that incorporates the path's log-signature.

The method states that over some interval $[r, s]$, we can approximate \cref{eq:ncde_integral} by
\begin{equation}
    z(s) \approx z(r) + \int^s_r \widehat{f}_\theta(t) \frac{\logsig^N_{r, s}(X)}{s - r} \dd t. 
    \label{eq:log_ode}
\end{equation}
\james{Can we add something about the form of $\widehat{f}$ here?} We see that the solution of the CDE from \cref{eq:ncde_integral} can be approximated by the ODE from \cref{eq:log_ode}. This then allows us to solve the Neural CDE model via computation of the log-signature terms followed by application of ODE solvers. 

In general, we will pick points $r_i$ such that $t_0 < r_0 < \ldots < r_n = t_n$, where the steps may potentially be larger than the discretisation of the data, and update
\begin{equation}
    z(r_{i+1}) = z(r_i) + \int^s_r \widehat{f}_\theta(t) \frac{\logsig^N_{r_i, r_{i+1}}(\Xx)}{r_{i+1} - r_i} \dd t.
\end{equation}
By utilising this approach, we can solve the Neural CDE equation using standard ODE solvers for multiple tools already exist \citep{rackauckas2017differentialequations, chen2018neural}. 

\subsection{Choice of control signal}
\james{Talk about how we have brushed over the control signal chat}

\subsection{Discussion}
\james{General points on CDEs, pros, cons, future work}

\subsection{Worked example}
\james{Could have a worked example here, not sure how possible it would be. I was thinking something like a brownian motion driving some response. We can show the conversion on to signatures and show how this drives and updates the neural CDE. This would help make it feel more tutorialey.} 

\subsection{Real-world examples}
Sepsis/MIMIC, long time series examples

==> Signatures IEEE/other/streams_old.tex <==
\section{\fontsize{14}{14}Streams, Controlled Differential Equations, and Signatures}
\label{sec:introduction}

The theory of rough paths is a foundational mathematical contribution that
extends Newton's and It\^{o}'s calculi modelling the interaction of systems
to much more complex and messy data streams. It has been recognised by
academic peers at a high level, e.g. Hairer's 2014 Fields Medal citation
notes: \textquotedblleft Building on the rough-path approach\ldots Hairer
was thus able to give, for the first time, a rigorous intrinsic meaning to
many SPDEs arising in physics.\textquotedblright\ A key idea is that it
measures the nonlinear interaction of an evolving system with simple test
systems and uses this \textquotedblleft description of the rough
system\textquotedblright\ to characterise the interaction of said system in
the context of interest. By measuring the simple interactions directly one
removes the need to sample or explore the system at a fine time resolution.
This top down approach allows a viable calculus of rough paths to be
developed. We explain how this work gives insight in modern data science. 

\subsection{Streams}

For this article and at its loosest, a stream is simply a multidimensional
system that has state and which evolves, and importantly, a system that can
be felt. By this I mean that it can interact in a dynamic way and has
effects that can be measured. A time series or the transactions in an order
book might represent a stream. The ever changing stock in a supermarket, the
interleaved flow of deliveries and of sales is a good example of a \emph{%
multimodal} stream. We do not want to preempt discussion of how to encode the
stream (for example how should one summarise the flow in the supermarket so
as to record information daily that is still sufficient to indicate the
contention between deliveries and consumption.Nor do we want to preclude
data that is only reasonably represented as a time series on such a fine
scale that it would be impossible to digitise it into a classical time
series. Think astronomical data.  

In this article one should think of a stream as a real world evolving object
that can be modelled as a time series on some ridiculously fine scale, but
which has effects which can be measured on normal timescales. The object is
still to be finally summarised, digitised, \ldots 

\subsection{Controlled differential equations}

The mathematical modelling of evolving systems via coupled differential
equations has a long and profound history; the calculus and the models were
developed at the same time. In Newton's work and language there were\
systems that evolved, with position (fluent) and direction (fluxion). They
interacted and there was a notion of a control (relate or dependent
variable; and correlate or independent variable) and he solved for the
evolution of the fluents.\footnote{Newton, Isaac, Methodus fluxionum et serierum infinitarum, 1671; The Method of Fluxions and Infinite Series; with Its Application to the Geometry of Curve-lines... Translated from the Author's Latin Original Not Yet Made Public. To which is Subjoin'd a Perpetual Comment Upon the Whole Work... by J. Colson. 1736.}

We use modern notation and language. Let $\ybold_{t}$ represent the
current state of a system and $\xbold_{t}=( x_{t}^{1},\ldots
,x_{t}^{n}) $ be a control that can influence the evolution of $%
\ybold_{t}$; then today it is natural to use a controlled
differential equation
\begin{eqnarray*}
d\ybold_{t} &=&\sum_{i}f^{i}( \ybold_{t})
dx_{t}^{i} \\
&=&\boldsymbol{f}( \ybold_{t}) d\xbold_{t}
\end{eqnarray*}%
to model the evolving response of $\ybold$ to $x$. In a simple case, 
$d\ybold_{t}$ represents the infinitesimal response of the system, $d%
\xbold_{t}$ infinitesimal control, and $\boldsymbol{f}$ the physics
that connects the control to the response. Numerical methods allow one to go
from such equations, and information about the control (e.g. the weights and
movements of the planets) to accurate simulations (e.g. of the moon).

Non-autonomous equations like 
\begin{equation*}
d\ybold_{t}=\boldsymbol{f}( \ybold_{t},\boldsymbol{t}%
) d\xbold_{t}+\boldsymbol{g}( \ybold_{t},%
\boldsymbol{t}) d\boldsymbol{t}
\end{equation*}%
look more general but they are not. We are already working with
multidimensional data, and by augmenting the state and control variables 
\begin{equation*}
\ybold_{t}\rightarrow ( \ybold_{t},\boldsymbol{t}%
) ,\ \ \xbold_{t}\rightarrow ( \xbold_{t},%
\boldsymbol{t}) 
\end{equation*}%
and modifying the physics%
\begin{eqnarray*}
d\ybold_{t} &=&\boldsymbol{f}( \ybold_{t},\boldsymbol{t}%
) d\xbold_{t}+\boldsymbol{g}( \ybold_{t},%
\boldsymbol{t}) d\boldsymbol{t} \\
d\boldsymbol{t} &\boldsymbol{=}&d\boldsymbol{t}
\end{eqnarray*}%
we may recast non-autonomous control problems as autonomous problems in an
enhanced state space. We may do the same with other more complex
intertwinings like $d\ybold_{t}=\boldsymbol{f}( \ybold%
_{t},\xbold_{t}) d\xbold_{t}$. It suffices to
understand the fundamental equation  
\begin{equation}
d\ybold_{t}=\boldsymbol{f}( \ybold_{t}) d%
\xbold_{t}  \label{eqn1:the fundamental controlled equation}
\end{equation}

Rough path theory tackles the generic question of how to understand this
fundamental equation in a way that scales smoothly from the smooth case to
the case where where the control $\xbold_{t}$ is multidimensional,
complex, and highly irregular on normal scales. It aims to give an accurate
macroscopic description of the response $\ybold_{t}$ over normal
scales even if  $\xbold_{t}$ is multidimensional, complex, and
highly irregular on these same scales. In the case where the physics is
regular and relatively smooth on this longer scale it suceeds in its aim.
For example, it gives deterministic meaning to the It\^{o}-Stratonovich
stochastic differential equations where $\xbold_{t}$ might be a
Brownian motion or a semimartingale and is certainly not differentiable and
amenable to classical calculus techniques. 

But these simple mathematical examples do not capture the breadth of the development. The P\&L (response) of an investment strategy (physics) applied to a financial market (the control), or a patient progressing in a hospital ward might be more interesting examples. Rough path theory substantially extends the scope (\ref{eqn1:the fundamental controlled equation}) of such equations going beyond It\^{o}'s stochastic differential equations. The rough calculus makes a radical break with the tradition of Newton and Riemann. Rather than focussing on the precise values of the control at particular times, which is not scalable as the path oscillates and becomes more complex, it looks at the path $\xbold_u$ over an interval $u \in [s, t) $ and tries to give a good enough description of $\xbold$ over the interval to predict well enough its effects on the response $\ybold$ at the end of the interval. We call this description the truncated signature and will say more below. Enough to say that it can give enough information to predict the main features of (the signature of) the response without probing into the microstructure of the control. Mathematically this is enough to give good mathematical meaning to the controlled differential equations driven by rough paths, but it also offers very practical numerical and top down approaches to summarising the complex stream of information in $\xbold_{[s, t)}$ into actionable forms that can be used to generate descriptions for $\ybold_{[s, t)}$.

The classical mathematical model for a path focuses on giving a value at
each time, rough path theory looks at giving approximate descriptions over
short time intervals of the "effects" of the stream or path on certain
prototype nonlinear systems. This second approach aligns much more closely
with wider human experience. A book is undoubtedly a stream or path of
letters. If we wanted to describe it, and particularly if we wanted to
summarise it, we would not think it very helpful to have every 100th letter.
On the other hand, brief synopses of sections could be much more valuable
(the first part of the book introduced a group of friends, the middle part
these individuals got separated and had different experiences, finally they
were reunited).

\subsection{Signatures and log-signatures}

Now we introduce quite precise mathematics that captures this top down
description of paths on normal scales. It is the essence of how one distils
from the information in control the key part needed to predict its effects.
Some of it will be very familiar to engineers (particularly those in
Robotics/Brocket) although the mathematics goes further. The key question to
address what information do I need to know about the control $\xbold%
_{[ s,t) }$ to compute or estimate $\ybold_{t}$ from the
state $\ybold_{s}$ at the beginning of the interval. This question
has a universal answer that does not depend on $f$ or $\ybold_{s}$.
Then what information is required, how to estimate $\ybold_{t}$
efficiently with this information. 

The answer to the first question is the signature of the control $%
\xbold_{[ s,t) }$while the answer to the second can be
built around the log signature. Consider the classical iterated approach of
Picard to solving a differential equation; lets formally apply iteration
here:
\begin{align}
    \begin{split}
        \ybold_{t} ={}& \ybold_s + \int_{s}^{t} f(\ybold_{u}) \dd \xbold_{u} 
    \end{split}\\
    \begin{split}
        ={}& \ybold_{s} + f(\ybold_s) \int_{s < u < t} \dd \xbold_u \\
             & + \int_{s < u_{1} < u_{2} < t} f^{\prime}(\ybold_{u_{1}}) f(\ybold_{u_{1}}) \dd \xbold_{u_{1}} \dd\xbold_{u_{2}}
    \end{split}\\
        ={}& \ybold_s + f(\ybold_{s}) \int_{s<u<t} \dd \xbold_{u} \\
           & + f^{\prime }(\ybold_{s}) f(\ybold_{s}) \int_{s < u_{1} < u_{2} < t} \dd \xbold_{u_{1}} \dd \xbold_{u_{2}} + \ldots 
    \end{align}
and if we continue we get two types of term - those that describe $%
\xbold$ over the interval and those that capture the function $f$
and the initial value $\ybold_{s}$ This suggests an answer to the
first question - an approximate description of $\xbold_{[
s,t) }$ is given by a sequence of tensor iterated integrals of the
stream called the signature:
\begin{align}
    S_{t} &:= S(\xbold_{[s, t)}) \\
    &:= \bigg(1, \int_{s < u < t} \dd \xbold_{u}, \int_{s < u_{1} < u_{2} <t} \dd \xbold_{u_{1}} \dd \xbold_{u_{2}}, \ldots \bigg)
\end{align}
However, it is not helpful to think of the signature as multiple integrals
as there is a challenge to computing them from our streams unless there is a
very fine digitisation. Importantly we easily observe that the signature $%
S_{t}$ satisfies its own differential equation:
\begin{equation*}
    \dd S_u = S_u \dd \xbold_u, \quad S_s = 1
\end{equation*}
In other words, conceptually we can compute the terms of the signature by
looking at the physical effect of the stream on this very simple nonlinear
exponential system and measure the response. We never need to digitise $x.$%
directly. In this way we can recover the first few terms in the signature
without ever exploring the microstructure of the control directly. This has
potential to substantially overcome the issues coming from the wild
behaviour of the control.

The log signature is a further step. .......

%%%%%%%%%%%%%%%%%%%%%%%%

% The mathematical modelling of evolving systems via coupled differential
% equations has a long and profound history; the calculus and the models were
% developed at the same time. If one lets $z_t$ represent the
% current state of a system and $X_t = (X_t^1, \ldots
% , X_t^n) $ be an external system that can influence the evolution
% then it is today natural to use a \textit{controlled differential equation}
% \begin{align}
%     \dd z_t &= \sum_{i} f^{i} (z_t) \dd X_t^i \\
%     &= f(z_t) \dd X_t
% \end{align}
% to model the evolution. In a simple case, $\dd z_t$ represents
% the response of the system, $\dd x_t$ the control, and $f$ the physics that connects the control and the response.
% Numerical methods allow one to go from such equations, and information about
% the external control (e.g. the weights and movements of the planets) to
% accurate simulations (e.g. of the moon). 

% It is tempting to think of time as special and consider non-autonomous
% equations 
% \begin{equation*}
%     \dd z_t = f (z_t, t) \dd X_t + g(z_t, t) \dd t
% \end{equation*}%
% but, because we are already working with multidimensional data one notes
% that by simply augmenting the state and control variables 
% \begin{align}
%     z_t &\rightarrow (z_t, t), \\
%     X_t &\rightarrow (X_t, t)
% \end{align}
% and modifying the physics
% \begin{align}
%     \dd z_t &= f(z_t, t) \dd X_t + g(z_t, t) \dd t \\ 
%     \dd t &= \dd t
% \end{align}
% we may recast non-autonomous control problems as autonomous problems in an
% enhanced state space. We may do the same with other more complex
% intertwinings like $\dd z_t = f(z_t, X_t) \dd X_t$.

% Rough path theory tackles the generic question of how to understand the
% fundamental equation linking evolution of a system and external controls   
% \begin{equation}
%     \dd z_t = f(z_t) \dd X_t
%     \label{eqn1:the fundamental controlled equation}
% \end{equation}
% in the case where we are interested in the response $z_t$
% over normal scales, the physics $f$ is reasonably smooth over
% normal scales, but where $X_t$ is multidimensional,
% complex, and irregular on normal scales. The P\&L of an investment strategy
% applied to a financial market, or a patient progressing in a hospital ward
% might be good examples. Rough path theory gives deterministic meaning to
% equations where $X_t$ is like a Brownian motion or is even
% wilder. It substantially extends the scope of such equations going beyond
% the calculus of It\^{o}. 

% This new calculus makes a radical break with the tradition of Newton and
% Riemann in an important way. Rather than focussing on the precise values of
% the control at particular times, which is not scalable as the path
% oscillates and becomes more complex, it looks at the path $X_u
% $ over an interval $u \in [s, t) $ and tries to give a good enough
% description of $X_t$ over the interval to predict well enough its
% effects on the response $z$ at the end of the interval. We call
% this description the truncated signature and will say more below. Enough to
% say that it can give enough information to predict the main features of (the
% signature of) the response without probing into the micro-structure of the
% control. Mathematically this is enough to give good mathematical meaning to
% the controlled differential equations driven by rough paths, but it also
% offers very practical numerical and top down approaches to summarising the
% complex stream of information in $X_{[s, t)}$ into
% actionable forms that can be used to generate descriptions for $z_{[s, t)}$. 

% The classical mathematical model for a path focuses on giving a value at
% each time, rough path theory looks at giving approximate descriptions over
% short time intervals of the "effects" of the stream or path on certain
% prototype nonlinear systems. This second approach aligns much more closely
% with wider human experience. A book is undoubtedly a stream or path of
% letters. If we wanted to describe it, and particularly if we wanted to
% summarise it, we would not think it very helpful to have every 100th letter.
% On the other hand, brief descriptions of the intervals of some interpretation
% could be much more valuable (the first part of the book introduced a group
% of friends, the middle part these individuals got separated and had
% different experiences, finally they were reunited).

% Using the signature, rough path theory faithfully describes complex
% sequential data in a top down way that avoids introducing a sampling
% parameterization and with a potentially massive dimension reduction. It can
% enhance existing data analysis tools and create a unified mathematical
% foundation for the high-order analysis of multimodal streamed data.


% \section{Can I get your signature?}
% We entered the competition Physionet 2019. The challenge was to build an online system that consumed the flow of medical information about a patient in the intensive care unit of a hospital, and from this irregular stream produced a warning of impending sepsis. Performance was measured via model submission that was tested locally on a large sample of unseen data by the competition organisers. There was a leader board, each team could submit 10 models over the months of the competition. There were over 100 teams. Our team -- ``Can I get you signature?'' -- utilised a mixture of techniques, with signatures forming a core component providing us with a necessary edge.

% We worked hard to do a professional job, but were actually pretty median in our ranking on the leader board after our first few efforts. To be honest we were a bit despondent. For performance reasons we were using the python package iisignature for training part of the signature calculations and our own python package esig for the inference and testing. We had failed to appreciate that the basis they used for describing log-signatures were different after level 2 and the numbers were completely incompatible at higher levels. Despite the name of our team, we had not been exploiting the signature! Once we discovered the error it was quickly corrected, and our next entry leapt to the top of the leader board; we stayed there for the rest of the competition (although others caught up) with this first ``correct'' entry. 

% This was the second time the path signature feature has lead to prizewinning work. The first time was in the hands of Ben Graham who combined signatures with his approaches to convolutional neural nets to win the ICDAR2013 online isolated Chinese character competition against strong competition. Lianwen Jin, and his team at South China University of Technology adopted Ben's methodology and created the state of the art input method for finger generated Chinese text entry for the mobile phone; their software has been adopted commercially and used on a regular basis by millions of people.

% The story of signatures is a mathematical one; their applicability to data comes from this mathematics. In both of the stories above the real impact came from the significant edge the signatures can give to the interpretation of data when used in combination with the other technologies of modern data science.

% The story we will tell is quite a slow burner, with many core ideas emerging over the last 30 years and now loosely summarised as ``the theory of rough paths''. However, the roots go further back. Core to rough path theory is the mathematical challenge of modelling evolving systems as they interact. The main tool we use to model continuous interactions is calculus. Already for Newton, his calculus provided the controlled differential equations that could be used to explain the interactions between planets. 


==> Signatures IEEE/sections/conclusion.tex <==
\section{Conclusion}

This paper attempts to provide a concise overview of some of the recent advances in the application of rough path theory to machine learning. Controlled differential equations (CDEs) are discussed as the key mathematical model to describe the interaction of a stream with a physical control system. The signature naturally arises in the description of the response produced by such interactions. The signature comes equipped with a variety of powerful properties rendering it an ideal feature map for streamed data. Next, we summarised recent advances in the symbiosis between deep learning and CDEs, studying the link with RNNs and culminating with the Neural CDE model. We concluded with a discussion on signature kernel methods, which are an alternative to deep learning methods.

\section*{Acknowledgements}

Terry Lyons’s contribution to this work is supported by the EPSRC program grant DataSig [grant number EP/S026347/1], and its project partners: in part by The Alan Turing Institute under the EPSRC grant EP/N510129/1, in part by The Alan Turing Institute’s Data Centric Engineering Programme under the Lloyd’s Register Foundation grant G0095, in part by The Alan Turing Institute’s Defence and Security Programme, funded by the UK Government, and in part by the Hong Kong Innovation and Technology Commission (InnoHK Project CIMDA).

==> Signatures IEEE/sections/interpretability.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/interpretability.png}
    \caption{Graphical depiction of the depth 1, 2, and 3 terms of the log-signature for a two-dimensional path $(X^1, X^2)$. \textbf{Left:} The first two depths that includes the change of the variables over the interval and the L\'evy area (shaded). \textbf{Middle and right:} Each plot only varies in a single depth 3 term with other terms being fixed. The middle plot sees varying area density along the $X^2$ axis, and the right along the $X^1$ axis.}
    \label{fig:interpretability}
\end{figure*}

\subsection{Interpretability}
Aside from being grounded in strong mathematical theory, the signature of a path also has geometric meaning. This is of particular interest when learning functions on data, since use of the signature can result in models that are interpretable and explainable. 

The left most plot in Figure \ref{fig:interpretability} contains the visualisations of both the depth 1 and 2 terms of the log-signature. The depth 1 terms are simply the change of the features over the interval; this can be seen directly via
\begin{equation*}
    \logsig^1_{s,t}(\boldsymbol{X}) = \int_{s < u < t} \dd \boldsymbol{X}_u = \boldsymbol{X}_t - \boldsymbol{X}_s = \Delta \mb{X}_{[s, t)}.
\end{equation*}

The depth 2 term is the signed area between the path and the chord joining the endpoints. This is also known as the \textit{L\'evy area} of the path; further examples can be found in \citet{chevyrev2016primer, morrill2020generalised}. 

There exist two more terms at depth 3, however, they are more difficult to visualize directly. However, consider the middle and right plots in \cref{fig:interpretability}. In each plot we draw three curves that differ only in their log-signature values at one of the two depth 3 terms, with the same depth 1 and 2 values.

The plot in the middle shows how one of the terms at depth 3 captures the distribution of the area along the $X^2$ axis. The right most plot demonstrates that the final term captures the extent to which the area has been loaded along the $X^{1}$ axis. 

\begin{example}[Interpretability of breathing data]
    To demonstrate how these features may be interpretable in the context of real data, consider a situation where we are seeking to predict stress from a persons respiratory data (a  problem where signatures have proved very successful). Consider each of the curves in \cref{fig:interpretability} to represent a single breath, with $X^1$ being time and $X^2$ the $\%$ expansion of a band located around the wearers chest that oscillates with breathing \citep[see][]{WESAD2018}.
    
    The values in the signature to depth 1 represent the total time of the breath ($\Delta X^1)$ and the difference in chest expansion from the start and end of the breath ($\Delta X^2$). The depth 2 term (the shaded area) approximates the volume of the inhalation. Finally, the depth 3 term can be seen to represent the sharpness of the inhale (\ref{fig:interpretability}, middle) and the extent to which the breath was a sharp inhale followed by a long exhale, or vice versa.
    (\ref{fig:interpretability}, right).
\end{example}

%% This example serves to demonstrate that the signature terms can be both highly interpretable, as well as highly extensible

Now that we have presented the main mathematical tools in the applications of rough path theory, we describe how these objects are applied in machine learning.




==> Signatures IEEE/sections/introduction.tex <==
\section*{Abstract}

This article provides a concise overview of some of the recent advances in the application of rough path theory to machine learning. Controlled differential equations (CDEs) are discussed as the key mathematical model to describe the interaction of a stream with a physical control system. A collection of iterated integrals known as the signature naturally arises in the description of the response produced by such interactions. The signature comes equipped with a variety of powerful properties rendering it an ideal feature map for streamed data. We summarise recent advances in the symbiosis between deep learning and CDEs, studying the link with RNNs and culminating with the Neural CDE model. We concluded with a discussion on signature kernel methods.

\section{Introduction}

% (TJL) an introduction needs to use vocabulary and concepts that resonate with the reader! These have to be primitive and of fundamental interest! What are they here? They cannot be stochastic analysis or SPDEs or citations of papers. We are not trying to justify rough path theory - we are trying to tell people what rough path theory does so they can get excited. In my view, we are not asking them to believe us that this stuff is useful, we are trying to give them the evidence so that they conclude this themselves. With hindsight I think the title is terrible and the self reference verges on narcissus. Can we find a direction to interest.

Complex and messy data streams (rough systems) are everywhere in our lives and come in profoundly different forms. They can take the form of a conversation, an electronic health record of a patient, the gravitational interaction of planets in our solar system, or the complex flow of traffic in a city. It is a profound and unfinished challenge to effectively model such streams, capture their ``meaning", and understand their interactions in a way that transcends the individual context. 

Rough path theory is an abstract mathematical tool-set that allows the modelling and analysis of evolving systems across a broad spectrum of use cases. It extends Newton's and It\^{o}'s calculus to model the interactions of complex and messy data streams. It has been influential within mathematics, in particular in stochastic analysis, as demonstrated by Hairer's 2014 Fields Medal citation notes: \textquotedblleft Building on the rough-path approach\ldots Hairer was thus able to give, for the first time, a rigorous intrinsic meaning to many Stochastic Partial Differential Equations (SPDEs) arising in physics.\textquotedblright. Like the mathematics of the number system, and the calculus of differential equations, the theory of rough paths exposes an aspect of the modelling of these streams that is separate from the context of interest (conversations, health records, solar system...).

A key insight in classical reservoir computing is that the trajectory of a dynamical system can be effectively described through its interaction with a 'black-box' non-linear system capable of storing information. In rough path theory, the dynamical system is replaced by a generic stream, the rough path, and the black-box by a simple and carefully chosen 'white-box' system, which fully describes the unparameterised stream \citep{hambly2010uniqueness}. The outcomes of these interactions build a \textquotedblleft structured description of the rough system\textquotedblright on a macroscopic scale. This mathematical description in terms of \textquotedblleft effects\textquotedblright is rich enough to characterise internal interactions and create a new calculus, without needing to directly determine its microscopic structure.

% Rough path analysis provides methodology and software that can be used effectively across widely different contexts. 

% The initial mathematical motivation for rough path theory came from It{\^o}'s successful calculus for modelling systems that interact with Brownian noise. By introducing a robust path-wise calculus capturing these stochastic interactions, rough paths theory answered many then open questions concerning classical It{\^o} analysis. 



% This theory provides powerful mathematical tools that can be used to design new tools -- such as the \emph{signature kernel} \citep{salvi2021signature} and \emph{neural rough differential equations} \citep{morrill2021neural} -- which are emerging as leading machine learning tools for sequential data. 


% It has been recognized by academic peers at a high level, e.g. Hairer's 2014 Fields Medal citation notes: \textquotedblleft Building on the rough-path approach\ldots Hairer was thus able to give, for the first time, a rigorous intrinsic meaning to many Stochastic Partial Differential Equations (SPDEs) arising in physics.\textquotedblright. 

% it describes the components of an evolving system (the rough paths) through their interaction with simple but carefully chosen test systems and uses these responses to build a \textquotedblleft description of the rough system\textquotedblright on a macroscopic scale without needing to directly determine its microscopic structure. 

% By measuring these specified nonlinear interactions directly over normal timescales one can adequately predict over normal timescales. One removes the need to sample or directly explore the system on finer time resolutions!

A traditional approach for handling time series is to record their values at regular intervals. Simple real-world examples demonstrate that this approach to describe streamed data is neither scalable nor practical. For example, consider the task of predicting the total CO2 emissions of a household over a month given the time series of their electricity consumption. The signals would need to be sampled significantly more often than 50 times a second to determine the power consumption. Rough path theory represents a radical change in the way one thinks mathematically about streamed data. It  summarises   the stream through a canonical sequence of coefficients, called the signature. The first three terms in the signature of the electrical stream provide sufficient information to compute the power consumption.

%A simple calculation shows that the first three iterated integrals, measured once in a month, provide already sufficient information about the stream to compute the power consumption over the month.

% Interactions between a (multivariate) time series and a system of interest are modelled by \emph{controlled differential equations} (CDEs) \citep{lyons2007differential}. The solution can then be expressed in terms of an object called the \emph{signature}. 



% There is a substantial conceptual difference between the signature and linear signal transforms such as Fourier series. 

The signature of a stream can be viewed as a generating function economically recording the effects of this stream on generic nonlinear systems. The geometer K.T. Chen used
this approach to understand multidimensional paths in the 1950s \citep{chen1954iterated}.

There are several substantial differences between the signature and classical signal processing transforms such as Fourier series and wavelets. One of the most significant is that Fourier series and wavelets are linear transformation and so treat the channels in a multimodal stream independently. As a result these transforms cannot capture information related to order of events occurring across the different channels. For example, regularly seeing the sequence: phone call, trade, price movement in the stream of office data monitoring a trader might be an indication of insider trading. Such occurrences
are straightforward to detect via a linear regression composed with the signature transform.
Modelling this signal using Fourier series or wavelets could be much more expensive: linearity
of these transforms imply that each channel must be resolved accurately enough to see the order of
events. 

The signature has the powerful property of being invariant to time-reparameterization of the underlying stream, which can have a dramatic effect on the complexity of certain challenges. In other words, the signature is a non-linear filter which removes the dependence on the sampling rate, while retaining all other information in the stream (in particular the order of events).


To sum up, rough path theory uses a top-down approach to summarise and digitise a stream. It uses a new feature set (signature) taken on longer timescales of interest, still capturing sufficient information to predict effects of the stream (the P\&Ls of different investment strategies for example). These summaries can be orders of magnitude more parsimonious without losing their effectiveness. This top-down methodology is in strong contrast to the bottom-up, finer and finer steps approach of classical integration and calculus.

Combined with state-of-the-art machine learning algorithms, the rough path approach for describing data streams has proved to be powerful for many real-world problems \cite{kidger2019deep}. For example, Hans Buehler says, in his ``2022 quant of the year award'' article: ``Signatures, thanks to their ability to converge to a stable result with a relatively small training dataset, proved perfectly suited to the task.'' % cite the buehler paper, the physionet challenge and chinese characters one. https://www.risk.net/awards/7926411/quant-of-the-year-hans-buehler

This article is organised as follows. Section \ref{sec:streams} introduces controlled differential equations (CDEs) and signatures. Section \ref{sec:nn_cdes} discusses how deep learning and rough path theory can be combined to learn the ``physics'' of a controlled system from observational data. Section \ref{sec:kernels} discusses signature kernel methods.


==> Signatures IEEE/sections/kernels.tex <==
\section{Signature kernels} \label{sec:kernels}

%We conclude by discussing another approach to learning with streams, based on signature kernels. 
Kernel methods have been shown to be efficient learning techniques in situations where inputs are non-Euclidean and the number of training instances is limited so that deep-learning-based techniques cannot be easily deployed \citep[see][for a detailed account on kernel methods in machine learning]{hofmann2008kernel}.  When the input data is sequential, the design of appropriate kernel functions is a notably challenging task. 

Consider a set $\Omega$ and let $\phi:\Omega\rightarrow H$ be a \emph{feature map} embedding elements of $\Omega$ into a Hilbert space $H$ (referred to as the \emph{feature space}).
% \begin{equation*}
%     \phi:\Omega\rightarrow E, \quad \psi:\Omega\rightarrow E^{\ast}.
% \end{equation*} 
% The pair of embeddings $(\phi,\psi)$ induces a \emph{kernel} $\kappa:\Omega\times \Omega\rightarrow\mathbb{R}$ defined for any $x,y \in \Omega$ as
% \begin{equation}
%     \kappa(x,y) = (\phi(x), \psi(y)),
% \end{equation}
% where $(\cdot,\cdot)$ is the natural pairing\footnote{Commonly, $E$ is assumed to be a Hilbert space, in which case $\psi=\phi$ and the pairing $(\cdot, \cdot) = \langle \cdot, \cdot \rangle$ is the inner product of the Hilbert space. However, the Hilbert space structure is not strictly necessary for the general picture.} \adeline{I would use the definition you put in the footnote since it is way more usual in the ML community and we do not need a lot of generality here} between the Banach space $E$ and its dual $E^*$.

For most of the popular kernels (RBF, Mat\'ern ...) $H$ is infinite dimensional and $\phi$ is either hard to compute or doesn't admit an explicit expression. Nonetheless, the kernel $\kappa$ can often be evaluated efficiently at any pair of points $x,y \in \Omega$ without referring back to the feature map. This property is known as  \emph{kernel trick}. 

Given a pair of $\Omega$-valued paths $\boldsymbol{X},\boldsymbol{Y}$, one can lift them both to two $H$-valued paths $\mathbb{X},\mathbb{Y}$ by means of the feature map $\phi$ as
\begin{equation*}
    \mathbb{X}_s = \phi(\boldsymbol{X}_s), \quad \mathbb{Y}_t=\phi(\boldsymbol{Y}_t).
\end{equation*}
% \adeline{Again, I do not understand why we need the liftings $\mathbb{X}$ and $\mathbb{Y}$ and do not work directly on the path $\boldsymbol{X}$ and $\boldsymbol{Y}$, which would make things simpler.}
Under the assumption that $\mathbb{X}$ and $\mathbb{Y}$ are continuous and have bounded variation, their signatures $\sig(\mathbb{X}), \sig(\mathbb{Y})$ are well defined as elements of $T((V))$. 
% It's not hard to prove that $T(V)$ is a Hilbert space and $T(V^*) = T(V)^*$ is its dual. 
Hence, the signature allows to turn a kernel $\kappa$ on $\Omega$ into a kernel $\kappa_{\text{sig}}$ on $\Omega$-valued paths defined as follows
\begin{equation*}
    \kappa_{\text{sig}}(\boldsymbol{X}_{s,s'},\boldsymbol{Y}_{t,t'}) = \left(\sig_{s,s'}(\mathbb{X}), \sig_{t,t'}(\mathbb{Y})\right).
\end{equation*}
We call $\kappa_{\text{sig}}$ the \emph{signature kernel} associated to the kernel $\kappa$. A natural question at this stage is: is there a kernel trick for $\kappa_{\text{sig}}$? 

The answer is positive and given by \citet[][Theorem 2.5]{salvi2021signature} who make a link between signature kernels and PDEs. In the simple case where the paths $\boldsymbol{X}, \boldsymbol{Y}$ are differentiable, the theorem states that $\kappa_{\text{sig}}(\boldsymbol{X}_{s,s'},\boldsymbol{Y}_{t,t'}) = U(s',t')$, where $U$ is the solution of the following linear hyperbolic PDE
\begin{equation}\label{eqn:PDE}
    \frac{\partial^2 U}{\partial p \partial q} = \kappa (\dot{\boldsymbol{X}}_p, \dot{\boldsymbol{Y}}_q)U
\end{equation}
with $U(s,\cdot)=U(\cdot,t)=1$, and where $\dot{\boldsymbol{X}}$ stands for the first time derivative of $\boldsymbol{X}$. The PDE \eqref{eqn:PDE} can be solved numerically using the finite differece schemes proposed in \citet{salvi2021signature} and implemented in the library \texttt{sigkernel}\footnote{\url{https://github.com/crispitagorico/sigkernel}}.

The availability of a kernel on paths allows to adapt standard kernel-based machine learning methods to the case of sequential data. It is straightforward to interface kernel estimators from \texttt{scikit-learn} \citep{pedregosa2011scikit} with \texttt{sigkernel} functionalities to build pipelines for time series classification (e.g. Support Vector Machine (SVM)), regression (e.g. Kernel-Ridge) or dimensionality reduction (e.g. kernel PCA) with no more than $10$ lines of code. 

For example, the table below shows classification accuracies (\%) on various UEA time series datasets \citep{bagnall2018uea} obtained by equipping a SVM classifier %\footnote{The hyperparameters of the SVM were selected by cross-validation. For more details see \citep{salvi2021signature}.} 
with different choices of kernels \footnote{When the time series are of the same length, standard kernels on $\mathbb{R}^d$ (Linear, RBF) can be used by stacking each channel into one single vector. When the series are not of the same length, other than the signature kernel, the \emph{global alignment kernel} \citep{cuturi2011fast} is a popular choice.}, including the signature kernel. As the results show, the signature kernel (SigKer) is systematically among the top $2$ classifiers across all the datasets (except for FingerMovements and UWaveGestureLibrary) and always outperforms its truncated counterpart (Sig$^N$). 

% \begin{table}
    \begin{center}
        \resizebox{.48\textwidth}{!}{
        \begin{tabular}{lccccc}
        \toprule
        \textbf{Datasets/Kernels} &
        Linear &
        RBF &
        GAK & 
        Sig$^N$ &
        SigKer \\
        \midrule
        ArticularyWordRecognition & 98.0 & 98.0 & 98.0 & 92.3 & \textbf{98.3}\\
        BasicMotions & 87.5 & 97.5 & 97.5 & 97.5 & \textbf{100.0} \\
        Cricket & 91.7 & 91.7 & \textbf{97.2} & 86.1 & \textbf{97.2}\\
        ERing & 92.2 & 92.2 & \textbf{93.7} & 84.1 & 93.3\\
        Libras & 73.9 & 77.2 & 79.0 & \textbf{81.7} & \textbf{81.7}\\
        NATOPS & 90.0 & 92.2 & 90.6 & 88.3 & \textbf{93.3}\\
        RacketSports & 76.9 & 78.3 & 84.2 & 80.2 & \textbf{84.9}\\
        FingerMovements & 57.0 & 60.0 & \textbf{61.0} & 51.0 & 58.0\\
        Heartbeat & 70.2 & 73.2 & 70.2 & 72.2 & \textbf{73.6}\\
        SelfRegulationSCP1 & 86.7 & 87.3 & \textbf{92.4} & 75.4 & 88.7\\
        UWaveGestureLibrary & 80.0 & \textbf{87.5} & \textbf{87.5} & 83.4 & 87.0\\
        \bottomrule
        \end{tabular}
    }
    \end{center}
    % \caption{Test set classification accuracy (in \%) on UEA multivariate time series datasets.}
    % \label{tab:svc}
% \end{table}

If a kernel is \emph{characteristic} \citep[see][for more details]{gretton2012kernel} and operates on the common support of two random variables, it can be used to define a notion of distance between random variables from finite collections of samples. This distance is commonly referred to as \emph{maximum mean discrepancy (MMD)} and can be used in practice to quantify the (dis)similarity between two datasets, hypothesis testing etc. 

\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\textwidth,trim={0 4.1cm 0 0},clip]{figures/particles.png}
\caption{\small Simulation of the trajectories traced by $20$ particles of an ideal gas in a $3$-d box under different thermodynamic conditions. Higher temperatures equate to a higher internal energy in the system which increases the number of collisions resulting in different large-scale dynamics of the gas.}
\label{fig:ideal_gas}
\end{figure*}

When the random variables are supported on path-space, they are called stochastic processes. Because the signature kernel is characteristic \citep[][Theorem 5.3]{chevyrev2018signature}, it allows to define a MMD on stochastic processes. Indeed, for any two compactly supported probability measures $\mathbb{P},\mathbb{Q}$ on path-space, one has the following representation of the MMD \citep[][Lemma 6]{gretton2012kernel}
\begin{align*}
    d_{\text{MMD}}(\mathbb{P}, \mathbb{Q})^2 &= \mathbb{E}_{(\boldsymbol{X},\boldsymbol{X}') \sim \mathbb{P} \times \mathbb{P}}[\kappa_{\text{sig}}(\boldsymbol{X},\boldsymbol{X}')] \\
    &- 2\mathbb{E}_{(\boldsymbol{X},\boldsymbol{Y})\sim \mathbb{P} \times \mathbb{Q}}[\kappa_{\text{sig}}(\boldsymbol{X},\boldsymbol{Y})]\\
    &+ \mathbb{E}_{(\boldsymbol{Y},\boldsymbol{Y}') \sim \mathbb{Q} \times \mathbb{Q}}[\kappa_{\text{sig}}(\boldsymbol{Y},\boldsymbol{Y}')].
\end{align*}
Given $M$ sample paths $\{\boldsymbol{X}^i\}_{i=1}^M \sim \mathbb{P}$ and $N$ sample paths $\{\boldsymbol{Y}^i\}_{i=1}^N \sim \mathbb{Q}$, the MMD can be computed in practice via the following unbiased estimator for $d_{\text{MMD}}(\mathbb{P}, \mathbb{Q})^2:$
\begin{align*}
    &\frac{1}{M(M-1)}  \sum_{i=1}^M\sum_{j\neq i}^M \kappa_{\text{sig}}(\boldsymbol{X}^i,\boldsymbol{X}^j) \\
    &- \frac{2}{MN}\sum_{i=1}^M\sum_{j=1}^N \kappa_{\text{sig}}(\boldsymbol{X}^i,\boldsymbol{Y}^j) \\
    &+ \frac{1}{N(N-1)}\sum_{i=1}^N\sum_{j\neq i}^N \kappa_{\text{sig}}(\boldsymbol{Y}^i,\boldsymbol{Y}^j).
\end{align*}
The characteristicness of $\kappa_{\text{sig}}$ makes the corresponding MMD an efficient statistics to distinguish two stochastic processes \citep[][Theorem 5]{gretton2012kernel}
\begin{equation*}
    d_{\text{MMD}}(\mathbb{P}, \mathbb{Q}) = 0 \iff \mathbb{P} = \mathbb{Q},
\end{equation*}
and consequently allows to build two-sample hypothesis tests for the null hypothesis
$H_0 : \mathbb{P} = \mathbb{Q}$ against the alternative $H_1: \mathbb{P} \neq \mathbb{Q}$.
The signature kernel has been applied in a variety of kernel-based contexts dealing with sequential data such as Gaussian Processes \citep{toth2020bayesian, lemercier2021siggpde} or Distribution Regression (DR) \citep{lemercier2021distribution, salvi2021higher}.

For example, in the context of DR, \citet{lemercier2021distribution} make use of the signature kernel to recover some thermodynamic properties of an ideal gas (e.g. the temperature) from the individual trajectories of its particles (see \Cref{fig:ideal_gas}). The complexity of the global dynamics of the gas depends on the environmental temperature ($T$) as well as on the radius of the particles ($r$). For a fixed temperature $T$, the larger the radius the higher the chance of collision between the particles. In the table below we report the DR results (MSE $10^{-2}$) of two experiments on simulated data: one where particles have a small radius (few collisions) and another where they have a bigger radius (many collisions). The performance of the signature kernel are superior but comparable to the ones produced by other models in the simpler setting (few collisions). However, in the presence of a high number of collisions, the signature kernel becomes more informative to retrieve the global temperature from local trajectories, while the performance from all other kernels deteriorates \citep[for additional experimental details see][]{lemercier2021distribution}.


\begin{center}
    \resizebox{.48\textwidth}{!}{
    \begin{tabular}{lcc}
    \toprule
    \textbf{Kernels/Regime} &
    Few collisions & Many collisions\\
    \midrule
    RBF & 3.08~(0.39) &  4.36~(0.64) \\
    Mat\'ern32 & 3.54~(0.48) &  4.12~(0.39)\\
    GAK & 2.85~(0.43) &  3.69~(0.36) \\
    SigKer &\textbf{1.31}~(0.34) &  \textbf{0.08}~(0.02)\\
    \bottomrule
    \end{tabular}
    }
\end{center}





==> Signatures IEEE/sections/ncdes.tex <==
\section{Deep learning and CDEs} \label{sec:nn_cdes}

Over the last few decades, neural networks have emerged as a spectacular new way of learning functional relationships from data. These functional relationships span a wide range of tasks such as computer vision or language generation, as well as based around the interpretation of streamed data. %In a somewhat quieter development, rough path theory has changed the way that one thinks about streamed data and controlled differential equations at a mathematical level. 

One of the exciting developments in this domain over the last couple of years has been the realisation that neural networks and differential equations are not competitors for describing functions on streams. Instead, there exists substantial synergy between the two models. This relationship was first stressed in the context of neural ordinary differential equations (neural ODEs), where neural networks are used as high capacity function approximators to learn ODEs \citep{chen2018neural}, and subsequently extended to other types of equations such as CDEs \citep{kidger2020neural, morrill2021neural}.

% \adeline{More details here on neural ODEs and the connection with Euler discretization schemes?}

In the next section, we outline how the mathematical theory introduced in \cref{sec:streams} can be used in tandem with neural networks to model functions on irregularly-sampled and partially observed time series, in the context of neural CDEs.

%This relationship is analogous to that found in the field of neural ordinary differential equations (neural ODEs), where neural networks are used as high capacity function approximators to learn ODEs \citep{chen2018neural}. \adeline{Introduce the idea of neural ODE which cannot be assumed to be known by everone.}

% Extending these ideas to rough paths and CDEs is an extension of the neural ODE since it allows to learn relationships between streams; a good example of this is learning functional relationships on time series -- an area where neural ODEs struggle.


% in which controlled differential equations are used to model functions on streams, but where the actual differential equation used (the physics) is learnt via a neural network. 

%\textcolor{blue}{The aim here is to contextualise the theory with respect to something the reader understands (RNNs). This will help to ground the ideas in something familiar before we introduce some new tools. }


\subsection{\fontsize{14}{14}Neural CDEs} \label{sec:ncdes}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/node_vs_ncde.png}
    \caption{Visual comparison of a Neural ODE vs a Neural CDE. \textbf{Left:} The Neural ODE encodes all information available to us at $t_0$ and propagates the hidden state forward in time, with no alterations based on future data. \textbf{Right:} The Neural CDE model has a mechanism to incorporate new data in continuous time.}
    \label{fig:node_vs_ncde}
\end{figure*}

We assume that we observe some data with their time-stamps: we are given a sequence 
\begin{equation*}\label{eq:def_data_sequence}
    \boldsymbol{x} = \big((t_1, x_1), \ldots, (t_T, x_T) \big),
\end{equation*}
where $t_i \in \reals$ are time-stamps such that $t_i < t_{i+1}$ and $x_i \in \reals^{d-1}$ are the features. The data may be both irregular (variable gaps between the $t_i$'s) and partially observed (not all features need to be measured at each $t_i$). 

To model the discrete data $\boldsymbol{x}$ using a CDE we must first formulate a continuous time embedding of the data, since the CDE evolves under the influence of a continuous time control $\boldsymbol{X}$. A sensible method is to use an interpolation of the data, typically such that $(t_j, \boldsymbol{x}_j) = \boldsymbol{X}_{t_j}$, $1 \leq j \leq T$; an in depth description of how one might do this is given by \citet{morrill2021neuralonline}. From now on, we denote by $\boldsymbol{X}$ the embedding of $\boldsymbol{x}$ as a continuous-time process.

%In this section we outline how the mathematical theory introduced in \cref{sec:streams} can be used in tandem with neural networks to model functions on such data, thanks to the \textit{neural controlled differential equation} (neural CDE) \citep{kidger2020neural, morrill2021neural, morrill2021neuralonline, bellot2021policy}%--- the rough path version of the neural ODE that applies to stream data. 

% can be used in practical applications to learn functions on real-world data processes. We introduce the \textit{neural controlled differential equation} (Neural CDE) which is a recently developed use case for rough path theory in machine learning applications \citep{kidger2020neural, morrill2021neural, morrill2021neuralonline, bellot2021policy}.

% Neural CDEs are an generalisation of the neural ordinary differential equation (neural ODE, \citet{chen2018neural}) that, as one might guess, models the data through use of a CDE rather than an ODE. This is an important generalisation as it allows the hidden state to evolve according to the behaviour of some underlying stream in continuous time. This cannot be accomplished by a neural ODE since it is uniquely determined by its initial condition; the neural ODE has no mechanism for incorporating data that arrives at later times. A high level visualisation of this difference is presented in \cref{fig:node_vs_ncde}. 

% The neural CDE model can be considered the continuous time equivalent of the recurrent neural network (RNN). In fact, the both the neural ODE and the RNN are just special cases of the neural CDE model \citep{kidger2020neural}.

%Equation \eqref{eq:continuous-rnn-cde} was a particular case of a neural CDE: 
 %\footnote{We opt for using $\boldsymbol{Z}_t$ rather than $\mb{Y}_t$ for the output here since it is usual to use the neural CDE to model a hidden state $\boldsymbol{Z}_t$ from which a linear map is applied to learn our output of interest $\mb{Y}_t$. The benefit of using a hidden state is that we can allow it to be of larger dimension than the output and thus it can carry more information.} 
The general idea of a neural CDE is to model a target hidden state $\boldsymbol{Z}_t$ which lives in $\reals^v$ by a CDE controlled by $\boldsymbol{X}$ of the form of \eqref{eq:cde}, in which we approximate the unknown vector field $\boldsymbol{f}$ with a neural network, denoted by $\boldsymbol{f}_\theta \colon \reals^v \rightarrow \reals^{v \times d}$. By letting $\zeta \in \reals^v$ be the initial condition, we say that the solution $\boldsymbol{Z}_t \in \reals^v$ to
\begin{equation}
    \dd \boldsymbol{Z}_t = \boldsymbol{f}_\theta (\boldsymbol{Z}_t) \dd \boldsymbol{X}_t, \quad \boldsymbol{Z}_{t_0} = \zeta,
    \label{eq:ncde}
\end{equation}
is the solution of a neural controlled differential equation. 
% \adeline{It is not clear here what is the output of the neural CDE and in which interval $t$ leaves} %In equation \eqref{eq:continuous-rnn-cde}, $f_\theta$ corresponds to a RNN but \eqref{eq:ncde} is more general and can correspond to any architecture.

The difference of a neural CDE compared with the neural ODE of \citet{chen2018neural} is simply that there is a $\dd \boldsymbol{X}_t$ rather than a $\dd t$ term. This modification is what enables the model to change continuously based on incoming data, since the path $\boldsymbol{X}_t$ adapts the dynamics of the system through the $\dd \boldsymbol{X}_t$ term.

Our goal now is to learn $\boldsymbol{f}_\theta$ from labelled training data such that the resulting CDE best models our problem of interest. However, it is not currently clear how this updating can be done, since we do now know how to update $\boldsymbol{Z}_t$ given $\boldsymbol{X}_t$. For this we will need to appeal to existing tools from rough path theory.

\subsubsection*{Training a neural CDE.}
First of all, for any data stream $\boldsymbol{X}$, we need to be able to compute the corresponding hidden state $\boldsymbol{Z}$, that is, to solve the neural CDE \eqref{eq:ncde}. If we instead had a neural ODE, where $\dd \boldsymbol{X}_t$ is $ \dd t$, then the method of solution is straightforward. We integrate the equation resulting in 
\begin{equation*}
    \boldsymbol{Z}_t = \boldsymbol{Z}_{t_0} + \int^t_{t_0} \boldsymbol{f}_\theta (\boldsymbol{Z}_u) \dd u
    \label{eq:node_integral}
\end{equation*}
and update $\boldsymbol{Z}_t$ using a standard integral solver. The integral form of the Neural CDE however is
\begin{equation*}
    \boldsymbol{Z}_t = \boldsymbol{Z}_{t_0} + \int^t_{t_0} \boldsymbol{f}_\theta (\boldsymbol{Z}_u) \dd \boldsymbol{X}_u.
    \label{eq:ncde_integral}
\end{equation*}

Our difficulty now lies in the fact that we need to integrate with respect to the multi-dimensional path control $\boldsymbol{X}_t$. Unsurprisingly, rough path theory holds the solution, and this solution is related to the log-signature of the path and more specifically to the log-ODE method discussed in Section \ref{sec:signatures}.

%As discussed in Section \ref{sec:signatures}, the log-signature is central to the study of CDEs. In fact, the log-signature can be thought of as precisely the information about a path that is required to solve any CDE that it drives. %This can be seen clearly from equation \cref{eq:taylor} where we see the (log-)signature terms arising out of the Taylor expansion of the CDE. 
%Specifically, we appeal to the log-ODE method \citep{castell1995efficient}, 

The log-ODE method describes how the solution of any CDE can be approximated by an ODE that incorporates the log-signature of the path. More precisely, it states that over an interval  $[s, t)$,
\begin{equation*}
    \boldsymbol{Z}_t \approx \boldsymbol{Z}_s + \int_s^t \widehat{\boldsymbol{f}}_\theta(\boldsymbol{Z}_u) \frac{\logsig^n_{s, t}(\boldsymbol{X})}{t - s} \dd u,
    %\label{eq:log_ode}
\end{equation*}
% \adeline{Are we sure that the log-signature is on $[s,t]$ here and not on $[s,u]$? If yes, why do we leave the log-signature inside the integral?}
where the vector field $\widehat{\boldsymbol f}_\theta : \mathbb{R}^v\rightarrow\mathbb{R}^v$ is defined for any $\boldsymbol y = (y_1,...,y_n) \in T^n(\mathbb{R}^d)$ as
\[\widehat{\boldsymbol{f}}_\theta(\boldsymbol{Z}_u) \boldsymbol y = \sum_{k=1}^n \boldsymbol f_\theta^k(\boldsymbol{Z}_u)y_k\]
where for any $k=1,...,n$ the functions $\boldsymbol f^k_\theta : \mathbb{R}^v \to L((\mathbb{R}^d)^{\otimes k}, \mathbb{R}^v)$ are defined recursively by
\begin{align*}
    \boldsymbol f^1_\theta = \boldsymbol f_\theta, \dots , \boldsymbol f^{(k+1)}_\theta = D(\boldsymbol f^k_\theta)\boldsymbol f_\theta,
\end{align*}
where $D(\cdot)$ denotes the Fr\'echet derivative. This allows us to evaluate the Neural CDE model via computation of the log-signature terms followed by application of ODE solvers. 
% \adeline{do we need so many details?}

To train the neural network, that is, to find the ``best'' set of parameters $\theta$ of the neural network $f_\theta$, we therefore proceed as follows. We pick points $r_i$ such that $t_0 < r_0 < \cdots < r_n = t_n$, where the steps may potentially be larger than the discretisation of the data, and update
\begin{align*}
    \boldsymbol{Z}_{r_{i+1}} &= \boldsymbol{Z}_{r_i} \\
    & \quad + \int^{r_{i+1}}_{r_i} \widehat{\boldsymbol{f}}_\theta(u) \frac{\logsig^N_{r_i, r_{i+1}}(\boldsymbol{X})}{r_{i+1} - r_i} \dd u.
\end{align*}
We then employ standard ODE solvers to update $\boldsymbol{Z}_t$, compare the final value against the true labels, and backpropagate the information to update $\boldsymbol{f}_\theta$ \citep{ chen2018neural}. 

We give in Figure \ref{fig:log-ode} a graphical depiction of this method.

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/log-ode.png}
    \caption{Pictorial description of the log-ode method used to solve a neural CDE. The data is converted onto a continuous embedding which is in turn converted into a collection of log-signatures that are used to update the hidden state.}
    \label{fig:log-ode}
\end{figure}


\subsubsection*{Performance.}

Neural CDEs have been shown to be highly performant across a range of benchmarks. \citet{kidger2020neural} show that the neural CDE outperforms similar ODE-benchmarks on a range of tasks on both performance metrics and memory usage. \citet{morrill2021neural} show that, by updating using higher degree log-signatures and longer steps, improvements in memory usage, training time, and model performance can all be achieved---this was verified on problems of length over 17,000. \citet{bellot2021policy} achieve state-of-the-art results using neural CDEs on counterfactual estimation tasks. A particular type of Neural CDEs are ones driven by Brownian motion, dubbed Neural SDEs. These models can serve as natural generative models for time series \citep{arribas2020sig, kidger2021neural}.

The examples considered were notably far reaching, ranging from the prediction of sepsis in ICUs to understanding the effect of Eurozone membership on the stream of current account deficits. They have also been successfully applied to datasets that are regular or irregular, fully or partially observed, and short problems to problems of long length (length $> 1000$). The ability to apply to problems of long length is facilitated by the rough log-ode update method that enables to trade length for additional log-signature terms making the method extremely useful for long-time series \citep{morrill2021neural}. 


To conclude, neural CDEs are a powerful tool for learning streams. In particular, they apply naturally to irregularly sampled and partially observed data. Indeed, the neural CDE interacts with the discrete data $\boldsymbol{x}$ through a continuous time embedding $\boldsymbol{X}$. This means that all data is placed on the same footing, be it irregular, partially observed, or both. This makes it a natural model for handling such non-regular data, which has posed a problem for previous models such as the RNN which expect data that is both regularly spaced and fully observed.
% They generalise other network models. Indeed, neural CDEs generalise neural ODEs since a $\dd t$ term is just a special case of $\dd \boldsymbol{X}_t$, where the path is a single dimension and increases linearly. It was also shown by \citet{kidger2020neural} that the recurrent neural network architecture (RNN) is a discretisation of a neural CDE; as such, the neural CDE is often called a continuous time equivalent of an RNN. \adeline{I would remove this point since it was discussed before}

Moreover, the neural CDE retains all the benefits of ODE modelling (adjoint method, continuously defined, error monitoring, ...). This is not true of many other similar models; for example, the ODE-RNN cannot operate using the memory efficient adjoint method of training  \citep[see][for more details]{kidger2020neural}.






==> Signatures IEEE/sections/rnns.tex <==
\subsection{Connection to RNNs}\label{sec:rnns}

Not only the connection between CDEs and neural networks allow to define new high-performance algorithms, but it also allows to better understand classical neural networks. In this subsection, we show that Recurrent Neural Networks (RNN), which are  very popular neural architectures for learning with  sequential data, may be reformulated in the language of rough path theory. This viewpoint is very rich; in particular, it allows to leverage the theory of CDEs and signatures to provide theoretical results on RNN, which is otherwise a very difficult endeavour. 

%In this section, we discuss the close link between RNN, CDEs and signatures, as presented by  \citet{fermanian2021framing}. This viewpoint yields as a byproduct generalization and stability bounds for a large class of RNN, which is a hard problem in deep learning.

We place ourselves in a supervised learning setting. The input data is a sample of $N$ i.i.d.~streams $\{\boldsymbol{x}^{(1)}, \dots,\boldsymbol{x}^{(N)}\}$, where each $\boldsymbol{x}^{(i)}$ is a stream as defined by \eqref{eq:def_data_sequence}. However, contrary to the previous section, we assume that all $\boldsymbol{x}^{(i)}$s are sampled on a regular partition: for any $1 \leq j \leq T$, we have $t_j = \nicefrac{j}{T}$. The outputs of the learning problem can be either labels (classification setting) or sequences (sequence-to-sequence setting). 


%is sampled at $T$ timepoints: $\boldsymbol{x}^{(i)} = (x^{(i)}_{1}, \dots, x^{(i)}_{T}) \in (\reals^d)^{T}$, $T\geq 1$. 

A (residual) recurrent neural network is defined by a sequence of hidden states $z_{1}, \dots, z_{T} \in\reals^v$, where, for $\boldsymbol{x}= (x_1, \dots, x_T)$ a generic data sample, for any $0 \leq j \leq T-1$,
\begin{equation} \label{eq:residual-rnn}
    z_{j+1} = z_{j} + \frac{1}{T}  f_\theta(z_{j}, x_{j+1}).
\end{equation}
At each time step $j$, the output of the network is $y_j = \psi(z_j)$, where $\psi$ is a linear function. The simplest choice for the function $f_\theta$ is the feedforward model (also known as Vanilla RNN), defined by
\begin{equation*}
    f_{\theta}(h, x) = \sigma(U h + V x + b),
\end{equation*}
where $\sigma$ is a nonlinear function applied element-wise (such as sigmoid or hyperbolic tangent), $U \in \reals^{v \times v}$ and $V \in \reals^{v \times d}$ are weight matrices, and $b \in \reals^{v}$ is the bias ($\theta$ is then a vector containing all the coefficients in $U$, $V$, and $b$). Note that the GRU \citep{Cho2014LearningPR} and LSTM \citep{hochreiter1997long} models can also be rewritten under the form \eqref{eq:residual-rnn}.

%To model our discrete data process using a CDE we must first formulate a continuous time embedding of the data, since the CDE evolves under the influence of a continuous time control. A sensible method is to use an interpolation of the data; an in depth description of how one might do this is given by \citep{morrill2021neuralonline}. 
We let $\boldsymbol{X}: [0,1] \to \reals^d$ denote the embedding of $\boldsymbol{x}$ (such that we have $\boldsymbol{x}_j = \boldsymbol{X}_{\nicefrac{j}{T}}$, $1 \leq j \leq T$). Following the neural ODE paradigm of \citet{chen2018neural}, the recursive equation \eqref{eq:residual-rnn} may be seen as an Euler discretization of the ODE
\begin{equation*}
    \dd \boldsymbol{Z}_t = f_\theta(\boldsymbol{Z}_t, \boldsymbol{X}_t)\dd t, \quad Z_0 =z_0, 
\end{equation*}
where $\boldsymbol{Z}$ is a continuous-time hidden state and $t \in [0,1]$. The output of the network at time $j$ is then $\psi(\boldsymbol{Z}_{\nicefrac{j}{T}})$. As mentioned before, by increasing the dimension of $\boldsymbol{Z}$, any ODE can be rewritten as a CDE of the form
\begin{equation*} \label{eq:continuous-rnn-cde}
    \dd \boldsymbol{Z}_t = \boldsymbol{f}_\theta(\boldsymbol{Z}_t) \dd \boldsymbol{X}_t.
\end{equation*}

An important property of the tensor algebra $T((\reals^d))$ introduced in Section \ref{sec:streams}, is that it can be equipped with a Hilbert structure \citep{Kiraly2016,salvi2021signature}, that is, with a scalar product denoted by $\langle \cdot, \cdot \rangle$. The following real-valued function
\begin{align*}
    \kappa: (\boldsymbol{X}, \boldsymbol{Y}) & \mapsto \langle \sig(\boldsymbol{X}), \sig(\boldsymbol{Y}) \rangle,
\end{align*}
is then well-defined, positive-definite, and called a kernel. The general idea of kernel methods is to map data to a high dimensional space so that linear methods may be used in this space, while being highly nonlinear in the original data \citep[see, e.g., ][]{scholkopf2018learning}. We refer to Section \ref{sec:kernels} for more details on kernel methods with signatures. Using a Taylor expansion of $\boldsymbol{Z}$, under some assumptions on the regularity of $\boldsymbol{f}_{\theta}$, it is then possible to show \citep[][Theorem 1]{fermanian2021framing} that there exists $\alpha(\theta) \in T((\reals^d))$ such that
\begin{equation*}   % \label{eq:hilbert-scalar-product}
    |y_T - \langle \alpha(\theta),\sig(\boldsymbol{X})  \rangle| \leq \frac{C}{T},
\end{equation*}
where $\alpha(\theta)$ depends only on the parameters of the RNN, $C$ is a constant, and $y_T$ is the final output of the RNN. In other words, if $g_\theta$ is the function that maps an input sequence $\boldsymbol{x}$ to the final output of the RNN (that is, $g_\theta(\boldsymbol{x}) = \psi(z_T)$), and if $\mathcal{H}$ is the reproducing kernel Hilbert space (RKHS) associated to $\kappa$, then $g_\theta \in \mathcal{H}$ at a $\mathcal{O}(\nicefrac{1}{T})$ error term.

This result allows to reinterpret the action of the recurrent network (RNN) as a scalar product in an (infinite-dimensional) Hilbert space, thereby framing the RNN as a kernel method. The key ingredients to obtain this Hilbert space are the Neural CDE model and the signature kernel.

A first consequence is that it gives natural generalization bounds under mild assumptions. For example, assume a binary classification problem, that is, we are given an i.i.d.~sample of $N$ random pairs of observations $(\boldsymbol{x}^{(i)}, \boldsymbol{y}^{(i)})$, where $\boldsymbol{y}^{(i)} \in \{-1, 1\}$.  In this context, the network outputs a real number $g_{\theta}(\boldsymbol{x})=\psi(z_T) \in \reals$ and the predicted class is $2 \cdot \boldsymbol{1}(g_{\theta}(\boldsymbol{x}) > 0) - 1$. The parameters $\theta$ of the RNN are fitted by empirical risk minimization using a loss function $\ell:\reals \times \reals \to \reals^{+}$, for example the logistic loss. The training loss is defined by
\begin{equation*}
   \widehat{\mathcal{R}}_{N}(\theta) = \frac{1}{N} \sum_{i=1}^N \ell \big(\boldsymbol{y}^{(i)}, g_{\theta}(\boldsymbol{x}^{(i)}) \big),
\end{equation*}
 and we let $\widehat{\theta}_N \in \textnormal{argmin }_{\theta \in \Theta } \widehat{\mathcal{R}}_N (\theta)$. Using the kernel approach described above, \citet[][Theorem 2]{fermanian2021framing} obtain the following informal result. Under some assumptions on its weight matrices, for a feedforward RNN, there exists a constant $B>0$ such that for any $ \theta$, $\| \alpha(\theta) \| \leq B$. Then with probability at least $1-\delta$,
    \begin{align*} %\label{eq:gen_bound_rnn_binary}
        &\mathbb{P}\big(\boldsymbol{y}g_{\widehat{\theta}_N}(\boldsymbol{x}) \leq 0| \mathcal{D}_N \big) \\
        & \quad \leq \widehat{\mathcal{R}}_N(\widehat{\theta}_N) + \frac{c_2}{T} + \frac{8 B K_{\ell} }{(1-L)\sqrt{N}} \\
        & \qquad + \frac{2BK_{\ell}}{1-L} \sqrt{\frac{\log(\nicefrac{1}{\delta})}{2N}}.
    \end{align*}

The term in $\mathcal{O}(\nicefrac{1}{T})$ comes from the continuous-time approximation, whereas the speed in $\nicefrac{1}{\sqrt{N}}$ is classical: the detour by CDEs provides a theoretical framework adapted to RNN, at the modest price of an additional $\mathcal{O}(\nicefrac{1}{T})$ term. 

In addition to providing a sound theoretical framework, framing deep learning in an RKHS provides a natural norm, which can be used for regularization. In our context, for two streams $\boldsymbol{x}$ and $\boldsymbol{y}$, we can bound the difference between the RNN outputs $g_\theta(\boldsymbol{x})$ and $g_\theta(\boldsymbol{y})$ by using the Cauchy-Schwartz inequality, as follows:
\begin{align*}
&|g_\theta(\boldsymbol{x})-g_\theta(\boldsymbol{y})| \\
& \quad \leq \frac{C}{T} + |\langle \alpha(\theta),S(\boldsymbol{X}) - S(\boldsymbol{Y})  \rangle| \\
& \quad \leq  \frac{C}{T} + \|S(\boldsymbol{X}) - S(\boldsymbol{Y}) \| \|\alpha(\theta)\|.
\end{align*}
If $\boldsymbol{x}$ and $\boldsymbol{y}$ are close, so are their embeddings $\boldsymbol{X}$ and $\boldsymbol{Y}$, and the term $\|S(\boldsymbol{X}) - S(\boldsymbol{Y}) \|$ is therefore small \citep[][Proposition 7.66]{friz2010multidimensional}. When $T$ is large, we see that the magnitude of $ \|\alpha(\theta)\|$ determines how close the predictions are. A natural training strategy to ensure stable predictions is then to penalize the problem by minimizing the loss $\widehat{\mathcal{R}}_n(\theta) + \lambda  \|\alpha(\theta)\|$.

% \adeline{I can cut from ``A first consequence of framing [...]'' to ``[...]at the modest price of an additional $\mathcal{O}(\nicefrac{1}{T})$ term'' and the paragraph still makes sense, depending on how long you want it to be.}

% \james{Length is fine at the moment, the plan is to send it as a draft to Robert Calderbank who is in charge of the journal, and get some feedback regarding style/length etc.}

To conclude, framing RNN as discretizations of CDEs is a powerful theoretical tool. It shows that the signature kernel appears naturally when analysing RNN. This kernel can also be used on its own to define new algorithms for data streams, which we now discuss.


==> Signatures IEEE/sections/streams.tex <==
\section{CDEs and signatures}\label{sec:streams}


% \subsection{Streams}

For this article a stream is a multidimensional evolving state that has effects. That is to say it can interact, over time intervals, with systems in transformative and measurable ways. 

To match with standard mathematical approaches, the reader might restrict attention to streams with an evolving state that can be recorded adequately as a smoothly sampled time series, denoted by $\boldsymbol{X}:[s,t) \rightarrow V$, where $V$ is a vector space, but they should allow that the sampling timescale may be orders of magnitude finer than the scales on which the effects they are interested in occur. Financial markets (micro-secs, days), astronomy (GHz, ms), speech (4kHz, .5 sec) and the power consumption of electric appliances (50Hz, minutes) all provide examples of this separation of timescales. In most cases, $V$ is chosen to be $\reals^d$, $d \geq 1$.

% The top down approach of rough path theory leads one to use Calculus and Controlled differential equations (CDEs) as the natural mathematical tools characterising streams and modelling their effects.

% \subsection{Streams}

% For this article, and at its loosest, a stream is simply a multidimensional evolving state that has effects. That is to say it can interact with (measurement) systems in a transformative way, with
% effects that evolve and can be measured. 

% To match with standard mathematical approaches, 

% We define a path to be a continuous function $\boldsymbol{X} : [0,1] \ \to \ \reals^{d}$, $d \geq 1$. Typically, $[0,1]$ corresponds to a time interval. Note that we will call $\boldsymbol{X}$ indifferently a path, a stream, or a time series. In practice, we observe $\boldsymbol{X}$ at a finite number of timesteps $0 \leq t_0 < \dots < t_n \leq 1$, which yields an ordered sequence of values $(x_1, \dots, x_n)$ such that $x_i = \boldsymbol{X}_{t_i}$.

% We denote by $\mathbf{x}$ the time series
% $$\mathbf{x} = \big((t_0, x_0), (t_1, x_1), \dots, (t_n, x_n)\big) \in (\reals^d)^n.$$ 

%$\mathbf{x}$ as an ordered collection of points $x_i \in \reals^{d-1}$ with corresponding time-stamps $t_0 < ... < t_n$, such that $t_i \in \mathbb{R}$ and
%$$\mathbf{x} = \big((t_0, x_0), (t_1, x_1), \dots, (t_n, x_n)\big) \in (\reals^d)^n.$$ 
%Let $\boldsymbol{X} : [t_0, t_n] \ \to \ \reals^d$ be some interpolation of the data such that $\boldsymbol{X}_{t_i} = (t_i, x_i)$  (piecewise linear, cubic splines etc.). More generally, we allow for $\boldsymbol{X}:[t_0, t_n] \rightarrow V$ to take its values on a $d$-dimensional Banach space $V$. 

% \begin{remark}
% In practice, the sampling timescale $\min_{i=1,...,n}\{t_i - t_{i-1}\}$ is often orders of magnitude finer than the scale at which the events of interest occur. Financial markets (micro-secs, days), Astronomy (GHz, ms), speech (4kHz, .5 sec) and the power consumption of electric appliances (50Hz, minutes) all provide examples of this separation of timescales. 
% \end{remark}

% The top down approach of rough path theory leads one to use Calculus and Controlled differential equations (CDEs) as the natural mathematical tools characterising streams and modelling their effects.

\subsection{CDEs}
The mathematical modelling of streams via controlled differential
equations has a long history. Already, in Newton's work and language there were\
systems that evolved, with position (fluent) and direction (fluxion). They
interacted and there was a notion of a control (relate or dependent
variable; and correlate or independent variable) and he solved for the
evolution of the fluents.\footnote{%
Newton, Isaac, Methodus fluxionum et serierum infinitarum, 1671; The Method
of Fluxions and Infinite Series; with Its Application to the Geometry of
Curve-lines... Translated from the Author's Latin Original Not Yet Made
Public. To which is Subjoin'd a Perpetual Comment Upon the Whole Work... by
J. Colson. 1736.}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/cover.png}
%     \caption{Template for ``things CDEs can model'' image. \adeline{this figure is never referred to in the text: should it be deleted?}}
%     \label{fig:cover}
% \end{figure*}

The language of controlled differential equations has matured. Consider first a conventional ordinary differential equation governed by a vector field $f$
\begin{eqnarray*}
\dd \boldsymbol{Y}_t = f\left( \boldsymbol{Y}_t\right) dt
\end{eqnarray*}
Such differential equation defines a flow; one can start the system at any point (the initial condition), but there are no other degrees of freedom for the dynamics. A controlled differential equation (CDE) is a differential equation where the dynamics, which are governed by $f$, can change according to an external stream of multimodal information $\boldsymbol X$ (called the control):
\begin{eqnarray}\label{eq:cde}
    \dd \boldsymbol{Y}_t = \boldsymbol{f}\left( \boldsymbol{Y}_t\right) \dd \boldsymbol{X}_t
\end{eqnarray}
Here, $\dd \boldsymbol{Y}_t$ represents the infinitesimal response of the system, $\dd \boldsymbol{X}_t$ the infinitesimal control, and $\boldsymbol{f}$ is a linear function mapping $\dd \boldsymbol{X}_t$ to vector fields on the $\boldsymbol{Y}$ space. CDEs also define a flow however there are infinitely many degrees of freedom.

% If $\boldsymbol{X}$ takes its values in $V$, and $\boldsymbol{Y}$ in $W$, then $\boldsymbol{f}: W \rightarrow \mathcal{L}(V, W)$ is the differential equation or vector field that governs the motion of $\boldsymbol{Y}$, where $\mathcal{L}(V,W)$ denotes the space of linear maps from $V$ to $W$. The linear map $ f(\boldsymbol{Y_u}): \boldsymbol{x} \mapsto f(\boldsymbol{Y_u}) \boldsymbol{x}$ is the physics that connects the control to the response. 
% Note that numerical methods developed over generations allow one to go from such equations to accurate simulations. %(e.g. the motion of the moon).




% Let $\boldsymbol{Y}_u \in \reals^{e}$ represent the current state of a system at time $u \in [0,1]$, and consider a control $\boldsymbol{X}_{u}=\left( X_{u}^{1},\ldots
% ,X_{u}^{d}\right) \in \reals^d$ that can influence the evolution of $\boldsymbol{Y}_{u}$; the dynamics linking $\boldsymbol X$ and $\boldsymbol Y$ can be modelled as a controlled differential equation (CDE)
% \begin{align} \label{eq:cde}
%     \dd \boldsymbol{Y}_{u} &=\boldsymbol{f}\left( \boldsymbol{Y}_{u}\right) \dd \boldsymbol{X}_{u} %= \sum_{i=1}^df^{i}\left( \boldsymbol{Y}_{u}\right) \dd X_{u}^{i}
% \end{align}
% Here, $\dd \boldsymbol{Y}_{u}$ represents the infinitesimal displacement of the system $\boldsymbol Y$ as a reaction to the infinitesimal displacement $\dd \boldsymbol{X}_{u}$ of the control $\boldsymbol X$ interacting with a control system determined by some vector fields $\boldsymbol{f}: \reals^{e} \rightarrow \mathcal{L}(\reals^{d}, \reals^{e})$, where $\mathcal{L}(\reals^{d}, \reals^{e})$ denotes the space of linear maps from $\reals^{d}$ to $\reals^{e}$. The linear map $ \boldsymbol f(\boldsymbol{Y}_u): x \mapsto \boldsymbol f(\boldsymbol{Y}_u) x$ represents the physics connecting the control to the response. Note that in \eqref{eq:cde} ``$\boldsymbol{f}(\boldsymbol{Y}_u) \dd \boldsymbol{X}_u$'' denotes a matrix-vector product, where $\boldsymbol{f}(\boldsymbol{Y}_u) \in \reals^{e \times d}$ and $\dd \boldsymbol{X}_u \in \reals^d$.
% Note that numerical methods developed over generations allow one to go from such equations to accurate simulations. %(e.g. the motion of the moon).

% Depending on the regularity assumptions on the control $\boldsymbol X$, \citep{kidger2020neural}, stochastic \citep{kidger2021neural} or a rough \citep{morrill2021neural} integral.
% Adeline: I think these citations very weird, it looks like the Riemann-Stieljes integral was invented in 2020... Moreover we have not talked yeat about integrals


% \subsubsection*{Other Forms of CDE}

% \begin{remark}
% % Note that non-autonomous equations like 
% %\begin{equation*}
% %\dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}_{u},u
% %\right) \dd \boldsymbol{X}_{u}+\boldsymbol{g}\left( \boldsymbol{Y}_{u},
% %u\right) \dd u
% %\end{equation*}%
% %such as Stochastic Differential Equations (SDEs) driven by a Brownian motion $\boldsymbol X$ fall under the above description. 
% Non-autonomous equations of the form
% \begin{equation*}
% \dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}_{u},u%
% \right) \dd \boldsymbol{X}_{u}+\boldsymbol{g}\left( \boldsymbol{Y}_{u},%
% u\right) \dd u
% \end{equation*}%
% look more general but they are not. Since $\boldsymbol{X}$ and $\boldsymbol{Y}$ are already multidimensional, by augmenting the state and control variables 
% \begin{equation*}
% \boldsymbol{Y}_{u}\rightarrow \left( \boldsymbol{Y}_{u},u%
% \right) ,\ \ \boldsymbol{X}_{u}\rightarrow \left( \boldsymbol{X}_{u},%
% u\right),
% \end{equation*}
% we may recast non-autonomous control problems as CDEs of the form \eqref{eq:cde} in an
% enhanced state space. We may do the same with other more complex intertwinings like 
% \begin{equation*}
%     \dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}%
% _{u},\boldsymbol{X}_{u}\right) \dd \boldsymbol{X}_{u}.
% \end{equation*} 
% % In conclusion, CDEs are very general and encapsulate, for example, stochastic differential equations (SDEs) or ordinary differential equations (ODEs).

% %understand the fundamental equation 
% %\begin{equation}
% %\dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}_{u}\right) \dd \boldsymbol{X}_{u}.  \label{eqn1:the fundamental controlled equation}
% %\end{equation}

% \end{remark}

\subsubsection*{Other Forms of CDE}
Non-autonomous equations like 
\begin{equation*}
\dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}_{u},\boldsymbol{u}%
\right) \dd \boldsymbol{X}_{u}+\boldsymbol{g}\left( \boldsymbol{Y}_{u},%
\boldsymbol{u}\right) \dd \boldsymbol{u}
\end{equation*}%
look more general but they are not. We are already working with
multidimensional data, and by augmenting the state and control variables 
\begin{equation*}
\boldsymbol{Y}_{u}\rightarrow \left( \boldsymbol{Y}_{u},\boldsymbol{u}%
\right) ,\ \ \boldsymbol{X}_{u}\rightarrow \left( \boldsymbol{X}_{u},%
\boldsymbol{u}\right) 
\end{equation*}%
and modifying the physics%
\begin{eqnarray*}
\dd \boldsymbol{Y}_{u} &=&\boldsymbol{f}\left( \boldsymbol{Y}_{u},\boldsymbol{u}%
\right) \dd \boldsymbol{X}_{u}+\boldsymbol{g}\left( \boldsymbol{Y}_{u},%
\boldsymbol{u}\right) \dd \boldsymbol{u} \\
\dd \boldsymbol{u} &\boldsymbol{=}&\dd \boldsymbol{u}
\end{eqnarray*}%
we may recast non-autonomous control problems as autonomous problems in an
enhanced state space. We may do the same with other more complex
intertwinings like $\dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}%
_{u},\boldsymbol{X}_{u}\right) \dd \boldsymbol{X}_{u}$. In conclusion, it suffices to
understand the fundamental equation 
\begin{equation*}
\dd \boldsymbol{Y}_{u}=\boldsymbol{f}\left( \boldsymbol{Y}_{u}\right) \dd \boldsymbol{X}_{u}.  \label{eqn1:the fundamental controlled equation}
\end{equation*}


\subsection{Describing a Stream with Signatures} \label{sec:signatures}

The simplest non-trivial CDE is probably the exponential, which for any $u \in [s, t)$, may be written informally as
\begin{equation}
\dd \boldsymbol{Y}_{u}=\boldsymbol{Y}_{u} \cdot \dd \boldsymbol{X}_{u},\quad 
\boldsymbol{Y}_{s}=1,  \label{eqn1:the signature equation}
\end{equation}%
where $\cdot$ denotes a multiplication to be defined later. Here, the evolution of $\boldsymbol{Y}$ exposes the effect of the stream $\boldsymbol{X}$ on the simplest non-linearity---multiplication. The measured response $\boldsymbol{Y}_{t}$ of this controlled system to the stream $\boldsymbol{X}_{u}$ over the interval $u\in \lbrack s,t)$ yields precise information about the stream over the interval. The geometer KT Chen used
this approach to understanding multimodal paths in the 1950s. The \emph{signature} $\sig_{s,t}(\boldsymbol{X})$ of the stream $\boldsymbol{X}$ on $[s,t)$ is defined as the response $\sig_{s,t}(\boldsymbol{X}):=\boldsymbol{Y}_{t}$. In other words, the signature $\sig_{s,t}(\boldsymbol{X})$ summarises the small-scale changes of $\boldsymbol{X}$ on $[s,t)$.

\subsubsection*{Tensors}

The equation \eqref{eqn1:the signature equation} implicitly requires that $%
\boldsymbol{Y}$ takes values in a space where one can multiply any element $%
\boldsymbol{Y}$ by any element $\boldsymbol{x}$ of $V$.
One gets the fullest description of $\boldsymbol{X}$ from the response $%
\boldsymbol{Y}$ if the algebra of the target space for the differential
equation imposes no other relations. The space generated by $V$ and a free
non-commutative multiplication operator is known as the tensor algebra. The
full signature is an element of this space, it is a sequence of tensors over
V; one of each degree. For those interested in details, we explain.

To make the exposition concrete, let $\boldsymbol{v_1},\boldsymbol{v_2},\ldots ,\boldsymbol{v_d} $ be a finite collection of letters (which we think of as an alphabet $A$) and suppose these letters are members of and form a basis for the linear space $V$. That is to say, every element $\boldsymbol{x}\in V$ is a unique linear combination $\sum_{i} x_i \boldsymbol{v_i} $ of letters in $A$. 

Now define $A^{\ast }$ to be the set of all words, including the empty word, whose
letters are drawn from $\boldsymbol{v_1},\boldsymbol{v_2},\ldots ,\boldsymbol{v_d}$. If $\boldsymbol{\varepsilon } $ is the empty word then 
\begin{align*}
A^{\ast }=\big\{& \boldsymbol{\varepsilon} ,\boldsymbol{v_1},\boldsymbol{v_2},\ldots, \boldsymbol{v_d}, \\
&\boldsymbol{v_1 v_1}, \boldsymbol{v_1 v_2},\ldots ,\boldsymbol{v_1v_d}, \\
&\boldsymbol{v_2v_1},\boldsymbol{v_2 v_2},\ldots \big\},
\end{align*}
and $T((V))$ is the vector space of all formal linear combinations of words
in $A^{\ast }$.  One can split this sum by the length of the word; one can write 
\begin{equation*}
\boldsymbol{y}=\sum_{\boldsymbol{w}\in A^*}y_{\boldsymbol w}\boldsymbol{w} \in T((V))
\end{equation*}
as
\begin{align*}
\boldsymbol{y}&= \overset{\text{degree 0}}{\vphantom{\sum_{A}}y_{\boldsymbol{\varepsilon }}\boldsymbol{\varepsilon }} + \overset{\text{degree 1}}{\sum_{
\boldsymbol{v_i}\in A}y_{\boldsymbol{v_i} }\boldsymbol{v_i}} \\
& \quad + \overset{\text{degree 2}}{\sum_{\boldsymbol{v_i,v_j}\in A}y_{\boldsymbol{v_iv_j}}%
 \boldsymbol{v_i v_j}} \\
 & \quad + \overset{\text{degree 3}}{\sum_{\boldsymbol{v_i,v_j,v_k}\in A}y_{\boldsymbol{v_iv_jv_k}} \boldsymbol{v_i v_j v_k}} + \cdots .
\end{align*}
The word of length zero yields a constant, the words of length one yield a
vector in $V$ while the words of length $n$ yield a tensor of degree $n$
over $V$. An element of $T((V))$ is an infinite sequence of tensors,
starting with a constant or 0 degree tensor, then a vector in $V$ or a $1$%
-tensor, then a matrix or a $2$-tensor, $3$-tensor, and so on.

The space $T((V))$ is an algebra; multiply words by concatenation 
\begin{align*}
    &( \boldsymbol{v_{i_1}}\ldots
\boldsymbol{v_{i_k}}) \left( \boldsymbol{v_{j_1}}\ldots \boldsymbol{v_{j_\ell}}\right) \\ 
& \quad = \boldsymbol{v_{i_1}}\ldots \boldsymbol{v_{i_k}}\boldsymbol{v_{j_1}}\ldots \boldsymbol{v_{j_\ell}},
\end{align*}

and extend their product to sums of words via the distributive
property. Multiplication is denoted by $\otimes $ for generic elements of $%
T\left( \left( V\right) \right) $ and sometimes for  concatenation of elements in $A$ for notational simplicity. The empty word $\boldsymbol{\varepsilon}$ is the unit and is  written as $\boldsymbol{1}$.

\emph{The signature of a path is an element of $T((V))$. It is a tensor of
every degree, or a coefficient associated to every word. One readily checks
that in the case where on some very fine scale }$\boldsymbol{X}$ is a
smooth path, and classical calculus applies, that the $n$-tensor term $%
\sig_{s,t}^{n}(\boldsymbol{X})$ in the signature is described recursively in terms
of the $(n-1)$-tensor term $\sig_{s,t}^{n-1}(\boldsymbol{X})$ without reference to the
higher order terms and
\begin{equation}
\sig_{s,t}^{n}(\boldsymbol{X})=\int_{u=s}^{t}\sig_{s,u}^{n-1}(\boldsymbol{X})\otimes \dd \boldsymbol{X}_{u}  \label{eqn3:iterated_integral_signature}
\end{equation}%
solves the differential equation (\ref{eqn1:the signature equation}) at
every tensor degree.

Back substitution in the formulation \eqref{eqn3:iterated_integral_signature} for the solution quickly reveals a second more popular expression for the
signature $\sig_{s,t}( \boldsymbol{X})$ in terms of iterated integral expansions.%
\begin{align*}
 \boldsymbol{1} & +\int_{s<u<t}\dd
\boldsymbol{X}_{u} \\
&  +\int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}_{u_{1}} \otimes \dd \boldsymbol{X}_{u_{2}} + \cdots .
\end{align*}%
Conceptually, the approach via effects offers a way to compute
the signature of a stream that, if non-linear sensors are available, is far
less computationally intensive than computing iterated integrals. The approach via
effects also allows one to deal with streams that have jumps in a much more
principled way.

\subsubsection*{The truncated signature}

%On the other hand, the full raw signature captures all possible behaviours needed to understand all possible systems driven by any stream. If a path has limited roughness, most of these scenarios will not be relevant and truncated signatures applied locally can provide a great intermediate feature set. 


Real numbers in a computer are traditionally truncated and represented using some version of IEEE Floating-Point Arithmetic. The tensor algebra T((V)) is managed similarly. By sending every word with more than $n$ letters, every tensor of degree greater than $n$, to zero, we get the truncated tensor algebra $T^{(n)}(V)$. 


An element of this truncated tensor algebra is a sequence of tensors of degree up to and including degree $n$. Multiplication and addition remain the same except that words of greater degree than $n$ that arise are set to zero and forgotten. 

The signature of the stream $\boldsymbol{X}_u,\ u\in [s,t)$ has tensor components of every positive integer degree $n$ and the number of degrees of freedom in a component grows exponentially with this degree! The complexity of $\boldsymbol{X}_u,\ u\in [s,t]$ determines the degree of the truncated signature needed to effectively describe $\boldsymbol{X}$. A path whose $n$ increments are drawn from an alphabet with $d$ letters already admits $d^n$ possibilities. 

If $V$ is finite dimensional and $d=\text{dim}(V)$ then the truncated algebra $T^{(n)}(V)$ has dimension $(d^{n+1} - 1)/(d-1)$; if $d>1$ the tensor of degree $n$ constitutes more than half the dimension of the entire truncated feature set. Because of this, one has the slightly surprising result that the computational complexity of multiplying two elements in the truncated tensor algebra is only logarithmically more than the cost of touching the data. This is in contrast to matrix multiplication which is much more expensive than the cost of touching the matrix. Numerical computation of signatures with well written code is primarily limited by memory bandwidth and is viable in quite high dimensions despite the exponential growth of the feature set.

The trick to using signatures to describe streams is to understand that they are very effective at describing oscillations that happen on a short time scale relative to matters of interest. Describing a stream effectively over a short interval may only require a few terms in the  signature and still be incredibly economical and accurate. However, shrinking the time intervals beyond this point becomes expensive because the data associated to lots of short time intervals is duplicate and irrelevant. This is the conundrum. 
The sweet spot is typically intermediate. Describing the stream over moderate length intervals using moderate depth truncated signatures can lead to dramatic efficiencies. 

\begin{example}[Electricity bill]
A good every day example is in the electricity bill. Electricity is delivered as a 2 dimensional time varying signal of voltage $V_t$ and changing charge $Q_t$. Both alternate, changing sign 50-60 times a second. 

From the perspective of the electric motor this short term description might be vital, but for many purposes the signal is adequately described by a single figure once a month - the total power consumed. In fact this total power consumption is the first significant term in the signature of the $(V_t,Q_t)$ path (it is a second order term - precisely the area and needs to be reported once in the month). This single nonlinear 2-truncated signature descriptor of the electric signal over the month describes the 129.8M oscillations well enough to allow prediction of CO$_2$ output etc. 

It is an interesting open exercise to identify the most parsimonious data store of truncated signatures over intermediate time intervals that is sufficiently information rich to allow identification of devices as they are switched on and off. The raw data is huge but not directly informative.
\end{example}

% \subsubsection*{NEXT}

% Multimodal streams are exponentially more complex than one dimensional streams.

% The equation equation (\ref{eqn1:the signature equation}) is well defined in 



% In the one dimensional case the solution is the exponential $\exp\left(\boldsymbol{X}_{t} - \boldsymbol{X}_{s} \right)$. 
% Rough path theory tackles the generic question of how to understand this
% fundamental equation in a way that scales smoothly from the smooth case to
% the case where where the control $\boldsymbol{X}_{t}$ is multidimensional,
% complex, and highly irregular on normal scales. It aims to give an accurate
% macroscopic description of the response $\boldsymbol{Y}_{t}$ over normal
% scales even if $\boldsymbol{X}_{t}$ is multidimensional, complex, and highly
% irregular on these same scales. In the case where the physics is regular and
% relatively smooth on this longer scale it suceeds in its aim. For example,
% it gives deterministic meaning to the It\^{o}-Stratonovich stochastic
% differential equations where $\boldsymbol{X}_{t}$ might be a Brownian motion
% or a semimartingale and is certainly not differentiable and amenable to
% classical calculus techniques.

% But these simple mathematical examples do not capture the breadth of the
% development. The P\&L (response) of an investment strategy (physics) applied
% to a financial market (the control), or a patient progressing in a hospital
% ward might be more interesting examples. Rough path theory substantially
% extends the scope (\ref{eqn1:the fundamental controlled equation}) of such
% equations going beyond It\^{o}'s stochastic differential equations. The
% rough calculus makes a radical break with the tradition of Newton and
% Riemann. Rather than focussing on the precise values of the control at
% particular times, which is not scalable as the path oscillates and becomes
% more complex, it looks at the path $\boldsymbol{X}_{u}$ over an interval $%
% u\in \left[ s,t\right) $ and tries to give a good enough description of $%
% \boldsymbol{X}$ over the interval to predict well enough its effects on the
% response $\boldsymbol{Y}$ at the end of the interval. We call this
% description the truncated signature and will say more below. Enough to say
% that it can give enough information to predict the main features of (the
% signature of) the response without probing into the microstructure of the
% control. Mathematically this is enough to give good mathematical meaning to
% the controlled differential equations driven by rough paths, but it also
% offers very practical numerical and top down approaches to summarising the
% complex stream of information in $\boldsymbol{X}_{\left[ s,t\right) }$ into
% actionable forms that can be used to generate descriptions for $\boldsymbol{Y%
% }_{\left[ s,t\right) }$.

% The classical mathematical model for a path focusses on giving a value at
% each time, rough path theory looks at giving approximate decriptions over
% short time intervals of the "effects" of the stream or path on certain
% prototype nonlinear systems. This second approach aligns much more closely
% with wider human experience. A book is undoubtedly a stream or path of
% letters. If we wanted to describe it, and particularly if we wanted to
% summarise it, we would not think it very helpful to have every 100th letter.
% On the other hand, brief synopses of sections could be much more valuable
% (the first part of the book introduced a group of friends, the middle part
% these individuals got separated and had different experiences, finally they
% were reunited).

% \subsection{Signatures and LogSignatures}

% Now we introduce quite precise mathematics that captures this top down
% description of paths on normal scales. It is the essence of how one distils
% from the information in control the key part needed to predict its effects.
% Some of it will be very familiar to engineers (particularly those in
% Robotics/Brocket) although the mathematics goes further. The key question to
% address what information do I need to know about the control $\boldsymbol{X}%
% _{\left[ s,t\right) }$ to compute or estimate $\boldsymbol{Y}_{t}$ from the
% state $\boldsymbol{Y}_{s}$ at the beginning of the interval. This question
% has a universal answer that does not depend on $f$ or $\boldsymbol{Y}_{s}$.
% Then what information is required, how to estimate $\boldsymbol{Y}_{t}$
% efficiently with this information.

% The answer to the first question is the signature of the control $%
% \boldsymbol{X}_{\left[ s,t\right) }$while the answer to the second can be
% built around the log-signature. Consider the classical iterated approach of
% Picard to solving a differential equation; lets formally apply iteration
% here:%
% \begin{eqnarray*}
% \boldsymbol{Y}_{t} &=&\boldsymbol{Y}_{s}+\int_{s}^{t}f\left( \boldsymbol{Y}%
% _{u}\right) \dd \boldsymbol{X}_{u} \\
% &=&\boldsymbol{Y}_{s}+f\left( \boldsymbol{Y}_{s}\right) \int_{s<u<t}\dd
% \boldsymbol{X}_{u}+\int_{s<u_{1}<u_{2}<t}f^{\prime }\left( \boldsymbol{Y}%
% _{u_{1}}\right) f\left( \boldsymbol{Y}_{u_{1}}\right) \dd \boldsymbol{X}%
% _{u_{1}}\dd \boldsymbol{X}_{u_{2}} \\
% &=&\boldsymbol{Y}_{s}+f\left( \boldsymbol{Y}_{s}\right) \int_{s<u<t}\dd
% \boldsymbol{X}_{u}+f^{\prime }\left( \boldsymbol{Y}_{s}\right) f\left( 
% \boldsymbol{Y}_{s}\right) \int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}_{u_{1}}\dd
% \boldsymbol{X}_{u_{2}}+\ldots 
% \end{eqnarray*}%
% and if we continue we get two types of term - those that describe $%
% \boldsymbol{X}$ over the interval and those that capture the frunction $f$
% and the initial value $\boldsymbol{Y}_{s}$ This suggests an answer to the
% first question - an approximate description of $\boldsymbol{X}_{\left[
% s,t\right) }$ is given by a squence of tensor iterated integrals of the
% stream called the signature:%
% \begin{equation*}
% S_{t}:=S\left( \boldsymbol{X}_{\left[ s,t\right) }\right) :=\left(
% 1,\int_{s<u<t}\dd \boldsymbol{X}_{u},\int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}%
% _{u_{1}}\dd \boldsymbol{X}_{u_{2}},\ldots \right) .
% \end{equation*}%
% However, it is not helpful to think of the signature as multiple integrals
% as there is a challenge to computing them from our streams unless there is a
% very fine digitisation. Importantly we easily observe that the signature $%
% S_{t}$ satisfies its own differential equation:%
% \begin{equation*}
% dS_{u}=S_{u}~\dd \boldsymbol{X}_{u},\ \ \ \ \ \ \ S_{s}=1
% \end{equation*}%
% In other words, conceptually we can compute the terms of the signature by
% looking at the physical effect of the stream on this very simple nonlinear
% exponential system and measure the response. We never need to digitise $x.$%
% directly. In this way we can recover the first few terms in the signature
% without ever exploring the microstructure of the control directly. This has
% potential to substantially overcome the issues coming from the wild
% behaviour of the control.

\subsubsection*{Signatures bring algorithmic improvement}

Signatures and controlled differential equations, when used to generate feature sets, remove parameterisation from a data stream, which can have a
dramatic effect on the complexity of certain challenges. We illustrate this with
a simple example which we call the insider trader problem. We first explain
the problem in the language of classical time series, and bucket data into
discrete time points.

\begin{example}[Insider trader problem]
Investigators have the records of several traders suspected of insider
trading, they would like to train a naive machine learnt function that they
could apply to other data to identify other suspected insider trader. Each
trader had associated with them a time series $\boldsymbol{x}:=\left\{ \left(
x_{i},y_{i},z_{i}\right) ,i=0,1,\ldots \right\} $ where $i$ represents the
minutes of the working day. Most times $x_{i},y_{i},z_{i}$ are all zero, but
(in this thought example) once a day the trader makes a short phone call; $%
x_{i}=1$ at the minute $i$ that the trader initiates her call. Once a day
the trader makes a trade in some asset; $y_{i}=1$ at the minute $i$ that the
trader initiates her trade. Once a day the
trader's asset has a value change; $z_{i}=1$ at the minute $i$ that the
asset price moves. There are $480$ minutes in a working day. The time series
has $3$ dimensions at each time or $1440$ dimensional in total. 

Suspect insider traders make the phone call, make the trade, and see the
price movement \emph{in that order}; any other order for these interactions
is not suspicious. Now consider a function $f$ that is $1$ if $i\leq j\leq k$
and zero otherwise and which identifies the suspects. A simple cubic
polynomial will do the job:%
\begin{equation*}
f\left( \boldsymbol{x}\right) :=\sum_{0\leq i<j<k<480}x_{i}y_{j}z_{k}
\end{equation*}%
but one immediately sees a problem; there are a huge number of ways that $%
i<j<k$ and even bigger complimentary set of non-suspicious triples. Training
to find the function $f$ cannot begin to get things correct unless it is
trained on most of these time series instances. $\left( 480\right) ^{3}$of
them. To see the pattern needs a huge amount of data and the situation gets
worse by several orders of magnitude if one refines the time scales.
Learning order information in multi-modal time series is extraordinarily
expensive.

However, adopting a signature approach transforms the situation. Let us
replace the discrete time series by a database of event tick data. The
database has three entries, $I$ the time of the phone call; $J$ the time of
the transaction; and $K$ the time of the asset price change. It is easy to
construct signatures from time stamped categorical tick data and the
complexity is $NC^{d}$ where $N$ is the number of ticks, $C$ is the number
of categories, and $d$ is the truncation degree of the signature. In our
case the number of ticks and categories is both $3$. Now, $f$ only depends
on the order and not the timing and so one knows that it can be realised as
a linear functional of the signature. It is actually a coefficient of the
signature truncated at degree $3$.

% \adeline{Add a citation to a paper that uses this approach? Terry: Unfortunately Hao did some work on noisy examples like this - it worked very well but she never wrote it up for publication}

So we have replaced our $1440$ dimensional time series representation of our
stream, to a $3^{4}$ or $81$ dimensional one and the function of interest is
a linear functional on this signature feature set. We have quite
dramatically reduced the amount of data required to learn the function. 
\end{example}

% Learning sequential information in multimodal data is extrodinarliy
% expensive, to the extent that it cannot be practically be done without
% filterning out the dependency of the time series on time parameterisation in
% some way and the algorithmic complexity increases with the time resolution.
% Going to a tick data representation, and using truncated signatures,
% completely removes the time resolution issue, allows irregular and complex
% data, creates fixed dimensional feature sets that are not influenced by
% sample rate or missing data, and can dramatically reduce the problem
% dimension so allowing learning from smaller datasets. 

\subsubsection*{The log-signature}

The signature is in some sense the exponential of the stream over a time interval---see Equation \eqref{eqn1:the signature equation}. It is the universal nonlinear response to the stream and any such response is well approximated by a linear projection of the signature. 

The log-signature summarises the stream in a somewhat different manner but plays an equally valuable role. It is a more concise descriptor of the stream over a time interval. It is a vector that is as easy to compute as the signature but has no redundancy. Polynomial functions in the log-signature have universality instead of the linear functions of the signature.

Its usefulness comes from the ease with which it can predict the effects of $\boldsymbol{X}$ on a a given non-linear system.  Consider again the equation 
\begin{eqnarray*}
\dd \boldsymbol{Y}_{u} &=&\sum_{i}f^{i}\left( \boldsymbol{Y}_{u}\right)
\dd X_{u}^{i} 
\end{eqnarray*}%
capturing the impact of $\boldsymbol{X}$ over a short interval of time $[s,t)$. Those interested in numerical solution of stochastic differential equations have for many years found it convenient to replace this system  with another \emph{time invariant} differential equation 
\begin{align*}
\dd\boldsymbol{y}_{v} = \boldsymbol{F}\left( \boldsymbol{y}_{v}\right)
\dd v, \quad v\in[0,1] 
\end{align*}
that captures the same net effect over $[0,1]$ to a high order of approximation as the controlled differential equation does over $[s,t)$. The choice of the differential equation (or vector field $\boldsymbol{F}$) depends on the stream over the interval $[0,t]$. But its solution can be delegated to classical ODE solvers. It is known as the log-ode method. It is usually one of the most efficient approaches to solving SDEs numerically. 

The choice of $\boldsymbol{F}$ is totally canonical and  is determined by the $f^i$ and is a linear combination of lie brackets of the $f^{i}$ determined by the \emph{log-signature} of $\boldsymbol{X}$ over the interval $[s,t)$. It is beyond this short note to explain this in detail, but should not be unfamiliar to those interested in control theory with knowledge of the the works of Brockett and Sussman, etc.
% \adeline{add a proper citation here.}

The log-signature is usually calculated by applying the power series for $\log(1+x)$ to the signature with the leading one removed. The log-signature is a linear combination of formal lie brackets $[\boldsymbol{v}_{i_1}, \ldots, [\boldsymbol{v}_{i_j},\boldsymbol{v}_{i_k}], \ldots,\boldsymbol{v}_{i_\ell}]$, which are easily translated to vector fields by substituting $f^i$ for $\boldsymbol{v}_{i}$. 
%It is not obvious that this approach works as it might have depended on the way the log-signature is expressed; in fact the target $F$ does not depend and the map is well defined as well as easy to implement.  
% and  of the The terms in the expansion of $\boldsymbol{F}$ give an alternative approach:
% \begin{align*}
% \boldsymbol{F} &= \sum_{i}f^{i}\int\limits_{s<u<t} \dd X^{i}_u \\
% &\quad +\sum_{i<j}[f^{i},f^{j}] \! \iint\limits_{s<u_1<u_2<t} \dd X^{i}_{u_1} \dd X^{j}_{u_2} -  \dd X^{j}_{u_2} \dd X^{i}_{u_1}\\
% & \quad + \cdots .
% \end{align*}
% \adeline{I do not understand where does this equation come from nor its meaning: is it a taylor expansion of the CDE? What's the link with the ``time-invariant'' differential equation?}
The first term in the log-signature is the increment of the stream in each coordinate, the second is the pairwise area. Higher order terms are easy to compute but require a choice of basis for the free Lie subalgebra of the Tensor algebra. There is a strong mathematical theory of these objects going back (among many others) to Hall, Schutzenberger, Ree, and Bourbaki \citep{ reutenauer2003free}. The software packages iisignature(PyPi) and esig(PyPi) both offer such calculations and the library libalgebra(C++, github) offers a broad range of related tools. 



% \subsection{Signatures} \label{sec:signatures}

% The simplest non-trivial CDE is probably the exponential, which for any $u \geq s$, may be written informally as
% \begin{equation}\label{eqn1:the signature equation}
% \dd \boldsymbol{Y}_{u}=\boldsymbol{Y}_{u} \otimes \dd \boldsymbol{X}_{u}, \quad 
% \boldsymbol{Y}_{s}=1,
% \end{equation}%
% where $\otimes$ denotes a multiplication to be defined later. Here, the evolution of $\boldsymbol{Y}$ exposes the effect of the stream $\boldsymbol{X}$ on the simplest non-linearity---multiplication. 
% The measured response $\boldsymbol{Y}_{t}$ of this controlled system to the stream $\boldsymbol{X}_{u}$ over the interval $u\in \lbrack s,t)$ yields precise information about the stream over the interval. 
% The geometer K.T. Chen used
% this approach to understand multidimensional paths in the 1950s \citep{chen1954iterated}. The signature $\sig(\boldsymbol{X}|_{[s,t)})$ of $\boldsymbol{X}$ over the interval $[s,t)$ is the solution of this exponential CDE:
% \begin{equation}\label{eqn:sig}
%     \boldsymbol{Y}_{t}=\sig(\boldsymbol{X}|_{[s,t)}).
% \end{equation}
% In other words, the signature $\sig_{s,t}(\boldsymbol{X})$ summarises the small-scale changes of $\boldsymbol{X}$ over $[s,t)$.

% The precise definition of the signature requires the introduction of the a vector space called the tensor algebra. %Readers primarily interested in machine learning applications should
% feel free to skip the next section.

% \subsubsection*{Tensor spaces.}

% \adeline{From a machine learning perspective, I think it is more natural to present elements of the tensor algebra as sequences of tensors rather than formal sums, because you then get a feature vector simply by flattening all tensors together. }
% The equation (\ref{eqn1:the signature equation}) implicitly requires that $%
% \boldsymbol{Y}$ takes values in a space where one can multiply any element $%
% \boldsymbol{Y}$ by any element $x$ of $V$.
% One gets the fullest description of $\boldsymbol{X}$ from the response $%
% \boldsymbol{Y}$ if the algebra of the target space for the differential
% equation imposes no other relations. The space generated by $V$ and a free
% non-commutative multiplication operator is known as the tensor algebra. The
% full signature is an element of this space, it is a sequence of tensors over
% V; one of each degree. For those interested in details, we explain.

% Let $A=\{v_1,v_2,\ldots ,v_d\}$ be an orthonormal basis of $V$. For any integer $k \geq 0$, $V^{\otimes k}$ is the vector space spanned by $k$-fold tensors
% \begin{equation*}
% v_{i_1} \otimes \dots \otimes v_{i_k}, \quad \text{with } i_1, \dots ,i_k \in \{1,\dots,d\}.
% \end{equation*}
% For example, $(\mathbb{R}^d)^{\otimes 2}=\mathbb{R}^{d \times d}$ is the space of all $d \times d$ matrices. Any element $x \in (\reals^d)^{\otimes k}$ can be decomposed as
% \[x = \sum_{i_1,\dots,i_k=1}^d x_{i_1,\dots,i_k} v_{i_1} \otimes \dots \otimes v_{i_k}, \]
%\begin{remark}
%Denoting the dual basis of $A^k$ by $\{
%v_{i_1}^* ... v_{i_k}^* \mid i_1,..,i_k \in \{1,..,d\}\}$ one can easily read off the coefficients of the above expansion:
%$$(v_{i_1}^*...v_{i_k}^*, y)=y_{i_1,...,i_k}.$$
%\end{remark}
% where $x_{i_1,\dots,i_k} \in \reals$.

% The tensor algebra $T(V)$ is the following direct sum of vector spaces
% \begin{equation}\label{eq:def_tensor_algebra}
%     T(V) = \mathbb{R} \oplus V \oplus V^{\otimes 2} \oplus ...
% \end{equation}
% Now, define $\Omega = \bigcup_{k \geq 0} A^k$ (with $A^0 = \{\varepsilon\}$ such that $\varepsilon$ spans $\reals$). Then, $T((\reals^d))$ is the vector space of all formal linear combinations of elements of $\Omega$. 
% whose
% letters are drawn from $v_1,v_2,\ldots ,v_d$. If $\boldsymbol{\varepsilon } $ is the empty word then 
% \begin{align*}
% A^{\ast }=\big\{& \boldsymbol{\varepsilon} ,v_1,v_2,\ldots, v_d, \boldsymbol{v_1 v_1}, \boldsymbol{v_1 v_2},\ldots ,\boldsymbol{v_1v_d}, \\
% &\boldsymbol{v_2v_1},\boldsymbol{v_2 v_2},\ldots \big\},
% \end{align*}
% and $T((V))$ is the vector space of all formal linear combinations of words
% in $A^{\ast }$.  
% One can split this sum by the length of the word; one can write 
% The space $T((\reals^d))$ is a vector space spanned by $\Omega = \bigcup_{k \geq 0} A^k$. Any element $\boldsymbol{y} \in T((\reals^d))$ has therefore an expansion of the form 
% \begin{align*} 
% \boldsymbol{y} &= \underbrace{y_{0}\varepsilon}_{\text{degree 0}} + \underbrace{\sum_{i=1}^d y_i v_i}_{\text{degree 1}} + \underbrace{\sum_{i_1, i_2=1}^d y_{i_1, i_2} v_{i_1} \otimes v_{i_2} }_{\text{degree 2}} \\
% & \quad + \underbrace{\sum_{i_1, i_2, i_3=1}^d y_{i_1, i_2, i_3} v_{i_1} \otimes v_{i_2} \otimes v_{i_3} }_{\text{degree 3}} + \cdots
% \end{align*}
% where
% \begin{align*}
% \boldsymbol{y}&= \overset{\text{degree 0}}{\vphantom{\sum_{A}}y_{\boldsymbol{\varepsilon }}\boldsymbol{\varepsilon }} + \overset{\text{degree 1}}{\sum_{
% v_i\in A}y_{v_i }v_i} + \overset{\text{degree 2}}{\sum_{\boldsymbol{v_i,v_j}\in A}y_{\boldsymbol{v_iv_j}}%
%  \boldsymbol{v_i v_j}} \\
%  & \quad + \overset{\text{degree 3}}{\sum_{\boldsymbol{v_i,v_j,v_k}\in A}y_{\boldsymbol{v_iv_jv_k}} \boldsymbol{v_i v_j v_k}} + \cdots .
% \end{align*}
% The word of length zero yields a constant, the words of length one yield a
% vector in $V$ while the words of length $n$ yield a tensor of degree $n$
% over $V$. 
% An element of $T((V))$ is an infinite sequence of tensors,
% starting with a constant or 0 degree tensor, then a vector in $V$ or a $1$%
% -tensor, then a matrix or a $2$-tensor, $3$-tensor, and so on.

% $T(V)$ is an algebra with the tensor product $\otimes$ defined as follows: for any $y, y' \in T(V)$
% \begin{equation*}
%     y \otimes y' = \sum_{k \geq 0}\sum_{j=0}^k y_j \otimes y'_{k-j}
% \end{equation*}
% The signature $\sig(\boldsymbol{X}|_{[s,t)})$ of a $V$-valued path $\boldsymbol{X}$ is an element of $T(V)$. Equation (\ref{eqn1:the signature equation}) can be written as follows in integral form 
% $$\sig(\boldsymbol{X}|_{[s,t)}) = 1 + \int_{s}^{t}\sig(\boldsymbol{X}|_{[s,u)})\otimes \dd \boldsymbol{X}_{u}.$$
% It follows that the signature can be expressed as the following collection of iterated integrals
% \begin{align*}
%     \sig(\boldsymbol{X}|_{[s,t)}) = 1 & + \int_{s<u<t}\dd\boldsymbol{X}_{u} \\
%     &+\int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}_{u_{1}} \otimes \dd \boldsymbol{X}_{u_{2}} \\
%     & \cdots  \\
%     & + \int_{s<u_1<\dots<u_k<t}\dd \boldsymbol{X}_{u_1} \otimes \dots \otimes \dd \boldsymbol{X}_{u_k} \\
%     & + \cdots
% \end{align*}

% multiply words by concatenation $( \boldsymbol{v_{i_1}}\ldots
% \boldsymbol{v_{i_k}}) \left( \boldsymbol{v_{j_1}}\ldots \boldsymbol{v_{j_\ell}}\right)= \boldsymbol{v_{i_1}}\ldots \boldsymbol{v_{i_k}}\boldsymbol{v_{j_1}}\ldots \boldsymbol{v_{j_\ell}}$ and extend their product to sums of words via the distributive
% property. Multiplication is denoted by $\otimes $ for generic elements of $%
% T\left( \left( V\right) \right) $ and sometimes for simple concatenation of elements in $A$ for notational simplicity. 
% Note that $\varepsilon$ is the unit and is often written as $\boldsymbol{1}$.

% \emph{The signature of a path is an element of $T((V))$. It is a tensor of
% every degree, or a coefficient associated to every word. One readily checks
% that in the case where on some very fine scale }$\boldsymbol{X}$ is a
% smooth path, and classical calculus applies, that the $n$-tensor term $%
% \sig_{s,t}^{n}(\boldsymbol{X})$ in the signature is described recursively in terms
% of the $n-1$-tensor term $\sig_{s,t}^{n-1}(\boldsymbol{X})$ without reference to the
% higher order terms and
% \begin{equation}
% \sig_{s,t}^{n}(\boldsymbol{X})=\int_{u=s}^{t}\sig_{s,u}^{n-1}(\boldsymbol{X})\otimes \dd \boldsymbol{X}_{u}  \label{eqn3:iterated_integral_signature}
% \end{equation}%
% solves the differential equation (\ref{eqn1:the signature equation}) at
% every tensor degree.

% Conceptually, the definition of the signature as solution to a differential equation offers a way to compute the signature of a stream that is far less computationally intensive than computing iterated integrals---provided non-linear sensors are available. \adeline{I do not understand the last part of the sentence: remove it?}
% The approach via effects also allows one to deal with streams that have jumps in a much more principled way.

% \subsubsection*{The truncated signature}

%On the other hand, the full raw signature captures all possible behaviours needed to understand all possible systems driven by any stream. If a path has limited roughness, most of these scenarios will not be relevant and truncated signatures applied locally can provide a great intermediate feature set. 

% \subsubsection*{Universal approximation property.}
% There is another algebraic structure, this time on the dual space $T((V^*))$, spanned by the elements of $\Omega^*$. The relevant product here is the shuffle product $\shuffle$, whose definition is not important as far as the present paper is concerned. What's important to note is that the linear functionals in $T((V^*))$, when restricted to the range of the signature, form an algebra of real-valued functions \citep[Theorem 2.15]{lyons2007differential} that contains constant functions and separate points \citep{hambly2010uniqueness}. Therefore, the celebrated \emph{Stone-Weierstrass theorem} applies and states that linear functionals acting on the signature are dense in the space of continuous functions on compact sets of paths. In other words, any continuous function on paths can be approximated uniformly well by linear regression on the terms of the signature. This renders the signature a universal approximator for doing inference on sequential data, justifying perhaps some of its success in machine learning applications. 

% \adeline{This paragraph is very cryptic for people who do not already know signatures: I would simply remove it and add later a comment on the `universal approximation'' property}

% \subsubsection*{The truncated signature.}

% To be computed and used in practice, the signature needs to be truncated at a finite degree $n \geq 0$, and we denote by $\sig^n(\boldsymbol{X}|_{[s,t)})$ the truncated signature at level $n$. The dimension of the truncated tensor algebra
% $$\text{dim}(T^n(V)) = \sum_{k \geq 0} d^k = \frac{d^{n+1}-1}{d-1}$$ 
% grows exponentially in $n$. 

% Effective numerical computation of signatures with well written code is viable in quite high dimensions despite this exponential growth. 


% Real numbers in a computer are traditionally truncated and represented using some version of IEEE Floating-Point Arithmetic. The tensor algebra T((V)) is managed similarly. By sending every word with more than $n$ letters, every tensor of degree greater than $n$, to zero, we get the truncated tensor algebra $T^{(n)}(V)$. 


% An element of this truncated tensor algebra is a sequence of tensors of degree up to and including degree $n$. Multiplication and addition remain the same except that words of greater degree than $n$ that arise are set to zero and forgotten. 

% The signature of the stream $\boldsymbol{X}_u,\ u\in [s,t)$ has tensor components of every positive integer degree $n$ and the number of degrees of freedom in a component grows exponentially with this degree! The complexity of $\boldsymbol{X}_u,\ u\in [s,t]$ determines the degree of the truncated signature needed to effectively describe $\boldsymbol{X}$. A path whose $n$ increments are drawn from an alphabet with $d$ letters already admits $d^n$ possibilities. 

% If $V$ is finite dimensional and $d=\text{dim}(V)$ then the truncated algebra $T^{(n)}(V)$ has dimension $(d^{n+1} - 1)/(d-1)$; if $d>1$ the tensor of degree $n$ constitutes more than half the dimension of the entire truncated feature set. Because of this, one has the slightly surprising result that the computational complexity of multiplying two elements in the truncated tensor algebra is only logarithmically more than the cost of touching the data. This is in contrast to matrix multiplication which is much more expensive than the cost of touching the matrix. Numerical computation of signatures with well written code is primarily limited by memory bandwidth and is viable in quite high dimensions despite the exponential growth of the feature set.

% The trick to using signatures for describing streams is to understand that they are very effective at describing oscillations that happen on a short time scale relative to matters of interest. Describing a stream effectively over a short interval may only require a few terms in the nonlinear signature and still be incredibly economical and accurate. However, shrinking the time intervals beyond this point becomes expensive because signatures associated to lots of short time intervals become duplicate and irrelevant. This is the conundrum. The sweet spot is typically intermediate: describing the stream over moderate length intervals using moderate depth truncated signatures can lead to dramatic efficiencies. 

% \begin{example}[Electricity bill]
% A good every day example is in the electricity bill. Electricity is delivered as a 2 dimensional time varying signal of voltage $V_t$ and changing charge $Q_t$, both alternate, changing sign 50-60 times a second. From the perspective of the electric motor this short term description might be vital, but for many purposes the signal is adequately described by a single figure once a month---the total power consumed. In fact this total power consumption is the first significant term in the signature of the $\boldsymbol{X}_t = (V_t,Q_t)$ path (it is a second order term, precisely the area, and needs to be reported once in the month). This single nonlinear 2-truncated signature descriptor of the electric signal over the month describes the 129.8M oscillations well enough to allow prediction of the output. It is an interesting open exercise to identify the most parsimonious data store of truncated signatures over intermediate time intervals that is sufficiently rich to allow identification of devices as they are switched on and off. 
% % The raw data is huge but not directly informative.
% \end{example}

% \subsubsection*{NEXT}

% Multimodal streams are exponentially more complex than one dimensional streams.

% The equation equation (\ref{eqn1:the signature equation}) is well defined in 



% In the one dimensional case the solution is the exponential $\exp\left(\boldsymbol{X}_{t} - \boldsymbol{X}_{s} \right)$. 
% Rough path theory tackles the generic question of how to understand this
% fundamental equation in a way that scales smoothly from the smooth case to
% the case where where the control $\boldsymbol{X}_{t}$ is multidimensional,
% complex, and highly irregular on normal scales. It aims to give an accurate
% macroscopic description of the response $\boldsymbol{Y}_{t}$ over normal
% scales even if $\boldsymbol{X}_{t}$ is multidimensional, complex, and highly
% irregular on these same scales. In the case where the physics is regular and
% relatively smooth on this longer scale it suceeds in its aim. For example,
% it gives deterministic meaning to the It\^{o}-Stratonovich stochastic
% differential equations where $\boldsymbol{X}_{t}$ might be a Brownian motion
% or a semimartingale and is certainly not differentiable and amenable to
% classical calculus techniques.

% But these simple mathematical examples do not capture the breadth of the
% development. The P\&L (response) of an investment strategy (physics) applied
% to a financial market (the control), or a patient progressing in a hospital
% ward might be more interesting examples. Rough path theory substantially
% extends the scope (\ref{eqn1:the fundamental controlled equation}) of such
% equations going beyond It\^{o}'s stochastic differential equations. The
% rough calculus makes a radical break with the tradition of Newton and
% Riemann. Rather than focussing on the precise values of the control at
% particular times, which is not scalable as the path oscillates and becomes
% more complex, it looks at the path $\boldsymbol{X}_{u}$ over an interval $%
% u\in \left[ s,t\right) $ and tries to give a good enough description of $%
% \boldsymbol{X}$ over the interval to predict well enough its effects on the
% response $\boldsymbol{Y}$ at the end of the interval. We call this
% description the truncated signature and will say more below. Enough to say
% that it can give enough information to predict the main features of (the
% signature of) the response without probing into the microstructure of the
% control. Mathematically this is enough to give good mathematical meaning to
% the controlled differential equations driven by rough paths, but it also
% offers very practical numerical and top down approaches to summarising the
% complex stream of information in $\boldsymbol{X}_{\left[ s,t\right) }$ into
% actionable forms that can be used to generate descriptions for $\boldsymbol{Y%
% }_{\left[ s,t\right) }$.

% The classical mathematical model for a path focusses on giving a value at
% each time, rough path theory looks at giving approximate decriptions over
% short time intervals of the "effects" of the stream or path on certain
% prototype nonlinear systems. This second approach aligns much more closely
% with wider human experience. A book is undoubtedly a stream or path of
% letters. If we wanted to describe it, and particularly if we wanted to
% summarise it, we would not think it very helpful to have every 100th letter.
% On the other hand, brief synopses of sections could be much more valuable
% (the first part of the book introduced a group of friends, the middle part
% these individuals got separated and had different experiences, finally they
% were reunited).

% \subsection{Signatures and LogSignatures}

% Now we introduce quite precise mathematics that captures this top down
% description of paths on normal scales. It is the essence of how one distils
% from the information in control the key part needed to predict its effects.
% Some of it will be very familiar to engineers (particularly those in
% Robotics/Brocket) although the mathematics goes further. The key question to
% address what information do I need to know about the control $\boldsymbol{X}%
% _{\left[ s,t\right) }$ to compute or estimate $\boldsymbol{Y}_{t}$ from the
% state $\boldsymbol{Y}_{s}$ at the beginning of the interval. This question
% has a universal answer that does not depend on $f$ or $\boldsymbol{Y}_{s}$.
% Then what information is required, how to estimate $\boldsymbol{Y}_{t}$
% efficiently with this information.

% The answer to the first question is the signature of the control $%
% \boldsymbol{X}_{\left[ s,t\right) }$while the answer to the second can be
% built around the log-signature. Consider the classical iterated approach of
% Picard to solving a differential equation; lets formally apply iteration
% here:%
% \begin{eqnarray*}
% \boldsymbol{Y}_{t} &=&\boldsymbol{Y}_{s}+\int_{s}^{t}f\left( \boldsymbol{Y}%
% _{u}\right) \dd \boldsymbol{X}_{u} \\
% &=&\boldsymbol{Y}_{s}+f\left( \boldsymbol{Y}_{s}\right) \int_{s<u<t}\dd
% \boldsymbol{X}_{u}+\int_{s<u_{1}<u_{2}<t}f^{\prime }\left( \boldsymbol{Y}%
% _{u_{1}}\right) f\left( \boldsymbol{Y}_{u_{1}}\right) \dd \boldsymbol{X}%
% _{u_{1}}\dd \boldsymbol{X}_{u_{2}} \\
% &=&\boldsymbol{Y}_{s}+f\left( \boldsymbol{Y}_{s}\right) \int_{s<u<t}\dd
% \boldsymbol{X}_{u}+f^{\prime }\left( \boldsymbol{Y}_{s}\right) f\left( 
% \boldsymbol{Y}_{s}\right) \int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}_{u_{1}}\dd
% \boldsymbol{X}_{u_{2}}+\ldots 
% \end{eqnarray*}%
% and if we continue we get two types of term - those that describe $%
% \boldsymbol{X}$ over the interval and those that capture the frunction $f$
% and the initial value $\boldsymbol{Y}_{s}$ This suggests an answer to the
% first question - an approximate description of $\boldsymbol{X}_{\left[
% s,t\right) }$ is given by a squence of tensor iterated integrals of the
% stream called the signature:%
% \begin{equation*}
% S_{t}:=S\left( \boldsymbol{X}_{\left[ s,t\right) }\right) :=\left(
% 1,\int_{s<u<t}\dd \boldsymbol{X}_{u},\int_{s<u_{1}<u_{2}<t}\dd \boldsymbol{X}%
% _{u_{1}}\dd \boldsymbol{X}_{u_{2}},\ldots \right) .
% \end{equation*}%
% However, it is not helpful to think of the signature as multiple integrals
% as there is a challenge to computing them from our streams unless there is a
% very fine digitisation. Importantly we easily observe that the signature $%
% S_{t}$ satisfies its own differential equation:%
% \begin{equation*}
% dS_{u}=S_{u}~\dd \boldsymbol{X}_{u},\ \ \ \ \ \ \ S_{s}=1
% \end{equation*}%
% In other words, conceptually we can compute the terms of the signature by
% looking at the physical effect of the stream on this very simple nonlinear
% exponential system and measure the response. We never need to digitise $x.$%
% directly. In this way we can recover the first few terms in the signature
% without ever exploring the microstructure of the control directly. This has
% potential to substantially overcome the issues coming from the wild
% behaviour of the control.

% \subsubsection*{Signatures bring algorithmic improvement}

% \subsubsection*{Invariance to time-reparametrization.}

% We illustrate with
% a simple example of insider trading. %We first explain the problem in the language of classical time series, and then bucket data into discrete time points.

% \begin{example}[Insider trading problem]
% Consider the following situation: investigators have the records of several traders suspected of insider trading, and they would like to build an algorithm that they could apply to new data to identify other suspected insider trader. Each
% trader had associated with them a time series $\boldsymbol{x}= \left\{ \left(
% x_{i},y_{i},z_{i}\right) ,i=0,1,\ldots \right\} $ where $i$ represents the
% minutes of the working day. At most times, $x_{i},y_{i},z_{i}$ are all zero, but
% (in this thought example) once a day the trader makes a short phone call; $%
% x_{i}=1$ at the minute $i$ that the trader initiates his call. Once a day
% the trader makes a trade in some asset; $y_{i}=1$ at the minute $i$ that the
% trader initiates his trade. Once a day the
% trader's asset has a value change; $z_{i}=1$ at the minute $i$ that the
% asset price moves. There are $480$ minutes in a working day. The time series
% has $3$ dimensions at each time or $1440$ dimensional in total. 

% Suspect insider traders make the phone call, make the trade, and see the
% price movement \emph{in that order}; any other order for these interactions
% is not suspicious. Now consider a function $f$ that is $1$ if $i\leq j\leq k$
% and zero otherwise and which identifies the suspects. A simple cubic
% polynomial will do the job:%
% \begin{equation*}
% f\left( x\right) =\sum_{0\leq i<j<k<480}x_{i}y_{j}z_{k}
% \end{equation*}%
% but one immediately sees a problem; there are a huge number of ways that $%
% i<j<k$ and an even bigger complimentary set of non-suspicious triples. Training
% to find the function $f$ cannot begin to get things correct unless it is
% trained on most of these time series instances ($480 ^{3}$of
% them). To see the pattern, one needs a huge amount of data and the situation gets
% worse by several orders of magnitude if one refines the time scales.
% In other words, learning order information in multi-modal time series is extraordinarily
% expensive.

% However, adopting a signature approach transforms the situation. Let us
% replace the discrete time series by a database of event tick data. The
% database has three entries: $I$ the time of the phone call, $J$ the time of
% the transaction, and $K$ the time of the asset price change. It is easy to
% construct signatures from time stamped categorical tick data and the
% complexity is $NC^{d}$ where $N$ is the number of ticks, $C$ is the number
% of categories, and $d$ is the truncation degree of the signature \adeline{It is not clear to me how such a signature is constructed: add some details on this, or a reference}. In our
% case the number of ticks and categories is both $3$. Now, $f$ only depends
% on the order and not the timing and so one knows that it can be realised as
% a linear functional of the signature. It is actually a coefficient of the
% signature truncated at degree $3$ \citep[Section 1.2]{bonnier2019deep}. \adeline{this reference does not add anything: in this paper nothing more is said from what is written here}
% \adeline{Add a citation to a paper that uses this approach? Terry: Unfortunately Hao did some work on noisy examples like this - it worked very well but she never wrote it up for publication}

% So we have replaced our $1440$ dimensional time series representation of our
% stream, to a $3^{4}$ or $81$ dimensional one and the function of interest is
% a linear functional on this signature feature set. We have quite
% dramatically reduced the amount of data required to learn the function. 
% \end{example}

% Learning sequential information in multimodal data is extrodinarliy
% expensive, to the extent that it cannot be practically be done without
% filterning out the dependency of the time series on time parameterisation in
% some way and the algorithmic complexity increases with the time resolution.
% Going to a tick data representation, and using truncated signatures,
% completely removes the time resolution issue, allows irregular and complex
% data, creates fixed dimensional feature sets that are not influenced by
% sample rate or missing data, and can dramatically reduce the problem
% dimension so allowing learning from smaller datasets. 

% \subsubsection*{The log-signature.}

% The signature is the exponential of the stream $\boldsymbol{X}$ over an interval, in the sense of equation \eqref{eqn1:the signature equation}. The \emph{log-signature}, denoted by $ \logsig_{s,t}(\boldsymbol{X})$ summarises the stream in a somewhat different manner but plays an equally valuable role. Formally, it is defined as the tensor logarithm of the signature; it is an element of the free Lie algebra in $d$ indeterminates \citep{reutenauer2003free, bourbaki2008lie}. Informally, it is a more concise descriptor of the stream in the sense that it removes the redudancy present in the signature \citep{chevyrev2016primer,liao2019learning}. Analogously to linear functional acting on the signature, polynomial functions acting on the log-signature have the universal approximation for continuous, real-valued functions on compact sets of paths. 


% It is the universal nonlinear response to the stream and any such response is well approximated by a linear projection of the signature. 

% Its usefulness comes from the ease with which it can predict the effects of $\boldsymbol{X}$ on a given non-linear system.  Consider again the CDE \eqref{eq:cde}
%\begin{equation*}
%    \dd \boldsymbol{Y}_{u} =\boldsymbol{f}\left( \boldsymbol{Y}_{u}\right) \dd \boldsymbol{X}_{u}%=\sum_{i=1}^df^{i}\left( \boldsymbol{Y}_{u}\right) \dd X_{u}^{i}
%\end{equation*}
% capturing the impact of $\boldsymbol{X}$ over a short interval of time $[s,t)$. Those interested in numerical solution of SDEs have for many years found it convenient to replace this system  with another \emph{time invariant} differential equation
% \[\dd\boldsymbol{y}_t = \boldsymbol{F}\left( \boldsymbol{y}_t\right)dt, \quad t\in [0,1],\]
% that captures the same net effect over $[0,1]$, to a high order of approximation, as the CDE (\ref{eq:cde}) does over $[s,t)$. The choice of vector field $\boldsymbol{F}$ depends on the stream $\boldsymbol X$, but its solution can be delegated to classical ODE solvers. It is known as the \emph{log-ode method}, and usually one of the most efficient approaches to solving SDEs numerically  \citep{castell1995efficient}. 

% The choice of $\boldsymbol{F}$ is totally canonical and  is determined by $\boldsymbol{f}$. Denoting by $f^i: \reals^{e} \to \reals$, $1 \leq i \leq d$, the columns of $\boldsymbol{f}$ such that
% \begin{equation*}
%     \dd \boldsymbol{Y}_{u} =\boldsymbol{f}\left( \boldsymbol{Y}_{u}\right) \dd \boldsymbol{X}_{u}=\sum_{i=1}^df^{i}\left( \boldsymbol{Y}_{u}\right) \dd X_{u}^{i},
% \end{equation*}
% then $\boldsymbol{F}$ consists of a linear combination of Lie brackets of the $f^{i}$ with coefficients determined by the terms of log-signature of $\boldsymbol{X}$ over the interval $[s,t)$. It is beyond the scope of this article to explain this in detail, but should not be unfamiliar to those interested in control theory \citep{sussmann1997300}.

% As mentioned earlier, the log-signature is usually calculated by applying the power series for $\log(1+x)$ to the signature with the leading one removed. The log-signature is a linear combination of formal lie brackets $[\ldots[a^{i},a^{j}]\ldots,a^{k}$, which are easily translated to vector fields by substituting $f^i$ for $a^i$. It is not obvious that this approach works as it might have depended on the way the log-signature is expressed; in fact the target $F$ does not depend and the map is well defined as well as easy to implement.  
% and  of the The terms in the expansion of $\boldsymbol{F}$ give an alternative approach:
% \begin{align*}
% \boldsymbol{F} &= \sum_{i}f^{i}\int\limits_{s<u<t} \dd X^{i}_u \\
% &\quad +\sum_{i<j}[f^{i},f^{j}] \! \iint\limits_{s<u_1<u_2<t} \dd X^{i}_{u_1} \dd X^{j}_{u_2} -  \dd X^{j}_{u_2} \dd X^{i}_{u_1}\\
% & \quad + \cdots .
% \end{align*}
% \adeline{I do not understand where does this equation come from nor its meaning: is it a taylor expansion of the CDE? What's the link with the ``time-invariant'' differential equation?}
% The first term in the log-signature is the increment of the stream in each coordinate, the second is the pairwise area. Higher order terms are easy to compute but require a choice of basis for the free Lie subalgebra of the Tensor algebra. There is a strong mathematical theory of these objects going back (among many others) to Hall, Schutzenberger, Ree, and Bourbaki \adeline{add proper citations}. 

% The software packages iisignature(PyPi) and esig(PyPi) both offer such calculations and the library libalgebra(C++, github) offers a broad range of related tools.  \adeline{idem: add citation to packages}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/interpretability.png}
    \caption{Graphical depiction of the depth 1, 2, and 3 terms of the log-signature for a two-dimensional path $(X^1, X^2)$. \textbf{Left:} The first two depths that includes the change of the variables over the interval and the L\'evy area (shaded). \textbf{Middle and right:} Each plot only varies in a single depth 3 term with other terms being fixed. The middle plot sees varying area density along the $X^2$ axis, and the right along the $X^1$ axis.}
    \label{fig:interpretability}
\end{figure*}

\subsubsection*{Geometric interpretation}

Aside from being grounded in strong mathematical theory, the signature of a path also has geometric meaning. This is of particular interest when learning functions on data, since use of the signature can result in models that are interpretable and explainable. 

The left most plot in Figure \ref{fig:interpretability} contains the visualisations of both the depth 1 and 2 terms of the log-signature. The depth 1 terms are simply the change of the features over the interval; this can be seen directly via
\begin{align*}
    \logsig^1_{s,t}(\boldsymbol{X}) 
    &= \int_{s < u < t} \dd \boldsymbol{X}_u \\
    &= \boldsymbol{X}_t - \boldsymbol{X}_s \\
    &= \Delta \mb{X}_{[s, t)}.
\end{align*}

The depth 2 term is the signed area between the path and the chord joining the endpoints. This is also known as the \textit{L\'evy area} of the path; further examples can be found in \citet{chevyrev2016primer}. 

There exist two more terms at depth 3, however, they are more difficult to visualize directly. However, consider the middle and right plots in \cref{fig:interpretability}. In each plot we draw three curves that differ only in their log-signature values at one of their depth 3 terms, with the same depth 1 and 2 values. The plot in the middle shows how one of the terms at depth 3 captures the distribution of the area along the $X^2$ axis. The right most plot demonstrates that the final term captures the extent to which the area has been loaded along the $X^{1}$ axis. 

\begin{example}[Interpretability of breathing data]
    To demonstrate how these features may be interpretable in the context of real data, consider a situation where we are seeking to predict stress from a persons respiratory data (a  problem where signatures have proved very successful). Consider each of the curves in \cref{fig:interpretability} to represent a single breath, with $X^1$ being time and $X^2$ the percentage expansion of a band located around the wearers chest that oscillates with breathing \citep[see][]{WESAD2018}.
    
    The values in the signature to depth 1 represent the total time of the breath ($\Delta X^1)$ and the difference in chest expansion from the start and end of the breath ($\Delta X^2$). The depth 2 term (the shaded area) approximates the volume of the inhalation. Finally, the depth 3 term can be seen to represent the sharpness of the inhale (\ref{fig:interpretability}, middle) and the extent to which the breath was a sharp inhale followed by a long exhale, or vice versa.
    (\ref{fig:interpretability}, right).
\end{example}

%% This example serves to demonstrate that the signature terms can be both highly interpretable, as well as highly extensible

Now that we have presented the main mathematical tools in applied rough path theory, we describe how these objects are applied in machine learning.




==> other/ncdes_old.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/node_vs_ncde.png}
%     \caption{Visual comparison on the RNN, ODE-RNN and Neural CDE methods. \textbf{Left:} the RNN updates the hidden state only at observation times and is undefined in-between. \textbf{Middle:} The ODE-RNN is defined between observations and modifies the hidden state at each observation. \textbf{Right:} The Neural CDE model first constructs a continuous time path control $\Xx$ resulting in a true continuous time interpretation of the hidden state.}
%     \label{fig:rnn_odernn_ncde}
% \end{figure*}

\subsection{Neural ODEs}
Neural ODEs seek to predict some output $y \in \reals^q$ from data $x \in \reals^d$ by learning a function $f_\theta \colon \reals^v \rightarrow \reals^v$ and linear maps $\ell^1_\theta \colon \reals^d \rightarrow \reals^v, \ell^2_\theta \colon \reals^v \rightarrow \reals^w$ such that 
\begin{multline}
    y \approx \ell^2_\theta(z_n) \;\; \text{where} \;\; z_{t} = z_{t_0} + \int^t_{t_0} f_\theta(z) \dd t \\ \text{and} \;\; z_0 = \ell^1_\theta(x).
    \label{eq:node}
\end{multline}
Neural ODEs provide us with an interface between the fields of machine learning and differential equation modelling. They allow us to combine modern tools from ODE research alongside the high flexibility and powerful function approximation properties from machine learning.

However, the definition as stated in \Cref{eq:node} cannot be straightforwardly applied to stream data. The key issue is that a Neural ODE defines an initial value problem; once $\theta$ has been learnt, the solution to \Cref{eq:node} is determined by the initial condition at $z_0$ with no direct mechanism for incorporating data that arrives later. 

To get around this issue, we must encode all information into the hidden state $z_0$ prior to running the Neural ODE model. This is an unnatural way to process sequential data and motivates the question of whether there is an extension that can process stream-like data, such as a time series.

\subsection{Neural CDEs}
The aforementioned issues with Neural ODEs can be naturally addressed by modelling the data with a CDE. After all, CDEs and rough path theory are really the study of how to incorporate (potentially complex and highly oscillatory) incoming signals to update some state. \james{Terry can you improve this sentence.}

Start by supposing we observe some discrete time series $\bx = \big((t_0, x_0), \ldots, (t_n, x_n) \big)$ with $t_i \in \reals$ denoting the timestamp of the observation vector $x_i \in (\reals \cup \{*\})^{d-1}$, where $*$ is used to denote that some information may be missing, and $t_0 < \ldots < t_n$. 

The first problem we have is that we (in general) observe a discrete data process but CDE theory relies on continuous time signals. Therefore, the first thing we must do is create a continuous time embedding of the discrete data process. Let $\Xx \colon [0, n] \rightarrow \reals^d$ be some interpolation of the data such that $\Xx(i) = (t_i, x_i)$, where `$=$' denotes equality up to missing data. We use the subscript $_\bx$ to highlight the dependence on the underlying discrete data process. The path $\Xx$ is often referred to as the \textit{control}. 

%% something about missing data
Our allowances for missing data may seem a little odd notationally, but keeping open the possibility for missing data is important. Often when observing real-world data we do not see all features simultaneously; for example, when patient laboratory tests are returned in an ICU we only see those that were requested by the doctor, with other information being missing. Our definition is also broad enough that it allows for the possibility of data that is irregularly sampled, another common property of real-world time series data. 

Issues of missingness and sampling irregularity are pervasive in real-world data and have historically posed a challenge when it comes to developing modelling frameworks. Recurrent neural networks (RNNs) have been the dominant modelling class for complex time series data across a range of domains \citep{sutskever2011generating,mikolov2010recurrent,graves2014towards}; however, they require regularly sampled and fully observed data, with standard workarounds being to divide the interval into equally-sized bins, and impute missing observations using averages. Such methods necessarily result in a loss of information.

%% something about how Neural Cdes fixes this problem

This time we take $f_\theta \colon \reals^v \rightarrow \reals^{v \times d}$. We then say the solution $z \in \reals^v$ to
\begin{equation}
    z_t = f_\theta(z_t) \dd \Xx \quad z_{t_0} = \zeta,
    \label{eq:ncde}
\end{equation}
is the solution of a \textit{neural controlled differential equation}. Here ``$f_\theta(z_s) \dd \Xx$'' denotes a matrix-vector product.

This can be written in the equivalent integral form
\begin{equation}
    \quad z_{t} = z_{t_0} + \int^t_{t_0} f_\theta(z_s) \dd \Xx.
    \label{eq:ncde_integral}
\end{equation}
from which the comparison to the Neural ODE from \cref{eq:node} becomes clear. We have simply replaced $\dd t \rightarrow \dd \Xx$. This seemingly minor modification is what enables our Neural CDE model to change continuously based on incoming data, since the path $\Xx$ adapts the dynamics of the system via the $\dd \Xx$ term. 

\subsection{The rough update}
Before proceeding, we must first understand how to evaluate the Neural CDE equation from \Cref{eq:ncde}. Whilst the modification of $\dd t \rightarrow \dd \Xx$ may seem a simple one, we are left now with a path integral for which the method of solution is not immediately clear.

Thankfully, the solution to this problem has already been addressed in the field of rough paths in the form of a method known as -- \textit{the log-ODE method} -- that can approximate the solution of any CDE equation to a corresponding ODE that incorporates the path's log-signature.

The method states that over some interval $[r, s]$, we can approximate \cref{eq:ncde_integral} by
\begin{equation}
    z(s) \approx z(r) + \int^s_r \widehat{f}_\theta(t) \frac{\logsig^N_{r, s}(X)}{s - r} \dd t. 
    \label{eq:log_ode}
\end{equation}
\james{Can we add something about the form of $\widehat{f}$ here?} We see that the solution of the CDE from \cref{eq:ncde_integral} can be approximated by the ODE from \cref{eq:log_ode}. This then allows us to solve the Neural CDE model via computation of the log-signature terms followed by application of ODE solvers. 

In general, we will pick points $r_i$ such that $t_0 < r_0 < \ldots < r_n = t_n$, where the steps may potentially be larger than the discretisation of the data, and update
\begin{equation}
    z(r_{i+1}) = z(r_i) + \int^s_r \widehat{f}_\theta(t) \frac{\logsig^N_{r_i, r_{i+1}}(\Xx)}{r_{i+1} - r_i} \dd t.
\end{equation}
By utilising this approach, we can solve the Neural CDE equation using standard ODE solvers for multiple tools already exist \citep{rackauckas2017differentialequations, chen2018neural}. 

\subsection{Choice of control signal}
\james{Talk about how we have brushed over the control signal chat}

\subsection{Discussion}
\james{General points on CDEs, pros, cons, future work}

\subsection{Worked example}
\james{Could have a worked example here, not sure how possible it would be. I was thinking something like a brownian motion driving some response. We can show the conversion on to signatures and show how this drives and updates the neural CDE. This would help make it feel more tutorialey.} 

\subsection{Real-world examples}
Sepsis/MIMIC, long time series examples

==> other/streams_old.tex <==
\section{\fontsize{14}{14}Streams, Controlled Differential Equations, and Signatures}
\label{sec:introduction}

The theory of rough paths is a foundational mathematical contribution that
extends Newton's and It\^{o}'s calculi modelling the interaction of systems
to much more complex and messy data streams. It has been recognised by
academic peers at a high level, e.g. Hairer's 2014 Fields Medal citation
notes: \textquotedblleft Building on the rough-path approach\ldots Hairer
was thus able to give, for the first time, a rigorous intrinsic meaning to
many SPDEs arising in physics.\textquotedblright\ A key idea is that it
measures the nonlinear interaction of an evolving system with simple test
systems and uses this \textquotedblleft description of the rough
system\textquotedblright\ to characterise the interaction of said system in
the context of interest. By measuring the simple interactions directly one
removes the need to sample or explore the system at a fine time resolution.
This top down approach allows a viable calculus of rough paths to be
developed. We explain how this work gives insight in modern data science. 

\subsection{Streams}

For this article and at its loosest, a stream is simply a multidimensional
system that has state and which evolves, and importantly, a system that can
be felt. By this I mean that it can interact in a dynamic way and has
effects that can be measured. A time series or the transactions in an order
book might represent a stream. The ever changing stock in a supermarket, the
interleaved flow of deliveries and of sales is a good example of a \emph{%
multimodal} stream. We do not want to preempt discussion of how to encode the
stream (for example how should one summarise the flow in the supermarket so
as to record information daily that is still sufficient to indicate the
contention between deliveries and consumption.Nor do we want to preclude
data that is only reasonably represented as a time series on such a fine
scale that it would be impossible to digitise it into a classical time
series. Think astronomical data.  

In this article one should think of a stream as a real world evolving object
that can be modelled as a time series on some ridiculously fine scale, but
which has effects which can be measured on normal timescales. The object is
still to be finally summarised, digitised, \ldots 

\subsection{Controlled differential equations}

The mathematical modelling of evolving systems via coupled differential
equations has a long and profound history; the calculus and the models were
developed at the same time. In Newton's work and language there were\
systems that evolved, with position (fluent) and direction (fluxion). They
interacted and there was a notion of a control (relate or dependent
variable; and correlate or independent variable) and he solved for the
evolution of the fluents.\footnote{Newton, Isaac, Methodus fluxionum et serierum infinitarum, 1671; The Method of Fluxions and Infinite Series; with Its Application to the Geometry of Curve-lines... Translated from the Author's Latin Original Not Yet Made Public. To which is Subjoin'd a Perpetual Comment Upon the Whole Work... by J. Colson. 1736.}

We use modern notation and language. Let $\ybold_{t}$ represent the
current state of a system and $\xbold_{t}=( x_{t}^{1},\ldots
,x_{t}^{n}) $ be a control that can influence the evolution of $%
\ybold_{t}$; then today it is natural to use a controlled
differential equation
\begin{eqnarray*}
d\ybold_{t} &=&\sum_{i}f^{i}( \ybold_{t})
dx_{t}^{i} \\
&=&\boldsymbol{f}( \ybold_{t}) d\xbold_{t}
\end{eqnarray*}%
to model the evolving response of $\ybold$ to $x$. In a simple case, 
$d\ybold_{t}$ represents the infinitesimal response of the system, $d%
\xbold_{t}$ infinitesimal control, and $\boldsymbol{f}$ the physics
that connects the control to the response. Numerical methods allow one to go
from such equations, and information about the control (e.g. the weights and
movements of the planets) to accurate simulations (e.g. of the moon).

Non-autonomous equations like 
\begin{equation*}
d\ybold_{t}=\boldsymbol{f}( \ybold_{t},\boldsymbol{t}%
) d\xbold_{t}+\boldsymbol{g}( \ybold_{t},%
\boldsymbol{t}) d\boldsymbol{t}
\end{equation*}%
look more general but they are not. We are already working with
multidimensional data, and by augmenting the state and control variables 
\begin{equation*}
\ybold_{t}\rightarrow ( \ybold_{t},\boldsymbol{t}%
) ,\ \ \xbold_{t}\rightarrow ( \xbold_{t},%
\boldsymbol{t}) 
\end{equation*}%
and modifying the physics%
\begin{eqnarray*}
d\ybold_{t} &=&\boldsymbol{f}( \ybold_{t},\boldsymbol{t}%
) d\xbold_{t}+\boldsymbol{g}( \ybold_{t},%
\boldsymbol{t}) d\boldsymbol{t} \\
d\boldsymbol{t} &\boldsymbol{=}&d\boldsymbol{t}
\end{eqnarray*}%
we may recast non-autonomous control problems as autonomous problems in an
enhanced state space. We may do the same with other more complex
intertwinings like $d\ybold_{t}=\boldsymbol{f}( \ybold%
_{t},\xbold_{t}) d\xbold_{t}$. It suffices to
understand the fundamental equation  
\begin{equation}
d\ybold_{t}=\boldsymbol{f}( \ybold_{t}) d%
\xbold_{t}  \label{eqn1:the fundamental controlled equation}
\end{equation}

Rough path theory tackles the generic question of how to understand this
fundamental equation in a way that scales smoothly from the smooth case to
the case where where the control $\xbold_{t}$ is multidimensional,
complex, and highly irregular on normal scales. It aims to give an accurate
macroscopic description of the response $\ybold_{t}$ over normal
scales even if  $\xbold_{t}$ is multidimensional, complex, and
highly irregular on these same scales. In the case where the physics is
regular and relatively smooth on this longer scale it suceeds in its aim.
For example, it gives deterministic meaning to the It\^{o}-Stratonovich
stochastic differential equations where $\xbold_{t}$ might be a
Brownian motion or a semimartingale and is certainly not differentiable and
amenable to classical calculus techniques. 

But these simple mathematical examples do not capture the breadth of the development. The P\&L (response) of an investment strategy (physics) applied to a financial market (the control), or a patient progressing in a hospital ward might be more interesting examples. Rough path theory substantially extends the scope (\ref{eqn1:the fundamental controlled equation}) of such equations going beyond It\^{o}'s stochastic differential equations. The rough calculus makes a radical break with the tradition of Newton and Riemann. Rather than focussing on the precise values of the control at particular times, which is not scalable as the path oscillates and becomes more complex, it looks at the path $\xbold_u$ over an interval $u \in [s, t) $ and tries to give a good enough description of $\xbold$ over the interval to predict well enough its effects on the response $\ybold$ at the end of the interval. We call this description the truncated signature and will say more below. Enough to say that it can give enough information to predict the main features of (the signature of) the response without probing into the microstructure of the control. Mathematically this is enough to give good mathematical meaning to the controlled differential equations driven by rough paths, but it also offers very practical numerical and top down approaches to summarising the complex stream of information in $\xbold_{[s, t)}$ into actionable forms that can be used to generate descriptions for $\ybold_{[s, t)}$.

The classical mathematical model for a path focuses on giving a value at
each time, rough path theory looks at giving approximate descriptions over
short time intervals of the "effects" of the stream or path on certain
prototype nonlinear systems. This second approach aligns much more closely
with wider human experience. A book is undoubtedly a stream or path of
letters. If we wanted to describe it, and particularly if we wanted to
summarise it, we would not think it very helpful to have every 100th letter.
On the other hand, brief synopses of sections could be much more valuable
(the first part of the book introduced a group of friends, the middle part
these individuals got separated and had different experiences, finally they
were reunited).

\subsection{Signatures and log-signatures}

Now we introduce quite precise mathematics that captures this top down
description of paths on normal scales. It is the essence of how one distils
from the information in control the key part needed to predict its effects.
Some of it will be very familiar to engineers (particularly those in
Robotics/Brocket) although the mathematics goes further. The key question to
address what information do I need to know about the control $\xbold%
_{[ s,t) }$ to compute or estimate $\ybold_{t}$ from the
state $\ybold_{s}$ at the beginning of the interval. This question
has a universal answer that does not depend on $f$ or $\ybold_{s}$.
Then what information is required, how to estimate $\ybold_{t}$
efficiently with this information. 

The answer to the first question is the signature of the control $%
\xbold_{[ s,t) }$while the answer to the second can be
built around the log signature. Consider the classical iterated approach of
Picard to solving a differential equation; lets formally apply iteration
here:
\begin{align}
    \begin{split}
        \ybold_{t} ={}& \ybold_s + \int_{s}^{t} f(\ybold_{u}) \dd \xbold_{u} 
    \end{split}\\
    \begin{split}
        ={}& \ybold_{s} + f(\ybold_s) \int_{s < u < t} \dd \xbold_u \\
             & + \int_{s < u_{1} < u_{2} < t} f^{\prime}(\ybold_{u_{1}}) f(\ybold_{u_{1}}) \dd \xbold_{u_{1}} \dd\xbold_{u_{2}}
    \end{split}\\
        ={}& \ybold_s + f(\ybold_{s}) \int_{s<u<t} \dd \xbold_{u} \\
           & + f^{\prime }(\ybold_{s}) f(\ybold_{s}) \int_{s < u_{1} < u_{2} < t} \dd \xbold_{u_{1}} \dd \xbold_{u_{2}} + \ldots 
    \end{align}
and if we continue we get two types of term - those that describe $%
\xbold$ over the interval and those that capture the function $f$
and the initial value $\ybold_{s}$ This suggests an answer to the
first question - an approximate description of $\xbold_{[
s,t) }$ is given by a sequence of tensor iterated integrals of the
stream called the signature:
\begin{align}
    S_{t} &:= S(\xbold_{[s, t)}) \\
    &:= \bigg(1, \int_{s < u < t} \dd \xbold_{u}, \int_{s < u_{1} < u_{2} <t} \dd \xbold_{u_{1}} \dd \xbold_{u_{2}}, \ldots \bigg)
\end{align}
However, it is not helpful to think of the signature as multiple integrals
as there is a challenge to computing them from our streams unless there is a
very fine digitisation. Importantly we easily observe that the signature $%
S_{t}$ satisfies its own differential equation:
\begin{equation*}
    \dd S_u = S_u \dd \xbold_u, \quad S_s = 1
\end{equation*}
In other words, conceptually we can compute the terms of the signature by
looking at the physical effect of the stream on this very simple nonlinear
exponential system and measure the response. We never need to digitise $x.$%
directly. In this way we can recover the first few terms in the signature
without ever exploring the microstructure of the control directly. This has
potential to substantially overcome the issues coming from the wild
behaviour of the control.

The log signature is a further step. .......

%%%%%%%%%%%%%%%%%%%%%%%%

% The mathematical modelling of evolving systems via coupled differential
% equations has a long and profound history; the calculus and the models were
% developed at the same time. If one lets $z_t$ represent the
% current state of a system and $X_t = (X_t^1, \ldots
% , X_t^n) $ be an external system that can influence the evolution
% then it is today natural to use a \textit{controlled differential equation}
% \begin{align}
%     \dd z_t &= \sum_{i} f^{i} (z_t) \dd X_t^i \\
%     &= f(z_t) \dd X_t
% \end{align}
% to model the evolution. In a simple case, $\dd z_t$ represents
% the response of the system, $\dd x_t$ the control, and $f$ the physics that connects the control and the response.
% Numerical methods allow one to go from such equations, and information about
% the external control (e.g. the weights and movements of the planets) to
% accurate simulations (e.g. of the moon). 

% It is tempting to think of time as special and consider non-autonomous
% equations 
% \begin{equation*}
%     \dd z_t = f (z_t, t) \dd X_t + g(z_t, t) \dd t
% \end{equation*}%
% but, because we are already working with multidimensional data one notes
% that by simply augmenting the state and control variables 
% \begin{align}
%     z_t &\rightarrow (z_t, t), \\
%     X_t &\rightarrow (X_t, t)
% \end{align}
% and modifying the physics
% \begin{align}
%     \dd z_t &= f(z_t, t) \dd X_t + g(z_t, t) \dd t \\ 
%     \dd t &= \dd t
% \end{align}
% we may recast non-autonomous control problems as autonomous problems in an
% enhanced state space. We may do the same with other more complex
% intertwinings like $\dd z_t = f(z_t, X_t) \dd X_t$.

% Rough path theory tackles the generic question of how to understand the
% fundamental equation linking evolution of a system and external controls   
% \begin{equation}
%     \dd z_t = f(z_t) \dd X_t
%     \label{eqn1:the fundamental controlled equation}
% \end{equation}
% in the case where we are interested in the response $z_t$
% over normal scales, the physics $f$ is reasonably smooth over
% normal scales, but where $X_t$ is multidimensional,
% complex, and irregular on normal scales. The P\&L of an investment strategy
% applied to a financial market, or a patient progressing in a hospital ward
% might be good examples. Rough path theory gives deterministic meaning to
% equations where $X_t$ is like a Brownian motion or is even
% wilder. It substantially extends the scope of such equations going beyond
% the calculus of It\^{o}. 

% This new calculus makes a radical break with the tradition of Newton and
% Riemann in an important way. Rather than focussing on the precise values of
% the control at particular times, which is not scalable as the path
% oscillates and becomes more complex, it looks at the path $X_u
% $ over an interval $u \in [s, t) $ and tries to give a good enough
% description of $X_t$ over the interval to predict well enough its
% effects on the response $z$ at the end of the interval. We call
% this description the truncated signature and will say more below. Enough to
% say that it can give enough information to predict the main features of (the
% signature of) the response without probing into the micro-structure of the
% control. Mathematically this is enough to give good mathematical meaning to
% the controlled differential equations driven by rough paths, but it also
% offers very practical numerical and top down approaches to summarising the
% complex stream of information in $X_{[s, t)}$ into
% actionable forms that can be used to generate descriptions for $z_{[s, t)}$. 

% The classical mathematical model for a path focuses on giving a value at
% each time, rough path theory looks at giving approximate descriptions over
% short time intervals of the "effects" of the stream or path on certain
% prototype nonlinear systems. This second approach aligns much more closely
% with wider human experience. A book is undoubtedly a stream or path of
% letters. If we wanted to describe it, and particularly if we wanted to
% summarise it, we would not think it very helpful to have every 100th letter.
% On the other hand, brief descriptions of the intervals of some interpretation
% could be much more valuable (the first part of the book introduced a group
% of friends, the middle part these individuals got separated and had
% different experiences, finally they were reunited).

% Using the signature, rough path theory faithfully describes complex
% sequential data in a top down way that avoids introducing a sampling
% parameterization and with a potentially massive dimension reduction. It can
% enhance existing data analysis tools and create a unified mathematical
% foundation for the high-order analysis of multimodal streamed data.


% \section{Can I get your signature?}
% We entered the competition Physionet 2019. The challenge was to build an online system that consumed the flow of medical information about a patient in the intensive care unit of a hospital, and from this irregular stream produced a warning of impending sepsis. Performance was measured via model submission that was tested locally on a large sample of unseen data by the competition organisers. There was a leader board, each team could submit 10 models over the months of the competition. There were over 100 teams. Our team -- ``Can I get you signature?'' -- utilised a mixture of techniques, with signatures forming a core component providing us with a necessary edge.

% We worked hard to do a professional job, but were actually pretty median in our ranking on the leader board after our first few efforts. To be honest we were a bit despondent. For performance reasons we were using the python package iisignature for training part of the signature calculations and our own python package esig for the inference and testing. We had failed to appreciate that the basis they used for describing log-signatures were different after level 2 and the numbers were completely incompatible at higher levels. Despite the name of our team, we had not been exploiting the signature! Once we discovered the error it was quickly corrected, and our next entry leapt to the top of the leader board; we stayed there for the rest of the competition (although others caught up) with this first ``correct'' entry. 

% This was the second time the path signature feature has lead to prizewinning work. The first time was in the hands of Ben Graham who combined signatures with his approaches to convolutional neural nets to win the ICDAR2013 online isolated Chinese character competition against strong competition. Lianwen Jin, and his team at South China University of Technology adopted Ben's methodology and created the state of the art input method for finger generated Chinese text entry for the mobile phone; their software has been adopted commercially and used on a regular basis by millions of people.

% The story of signatures is a mathematical one; their applicability to data comes from this mathematics. In both of the stories above the real impact came from the significant edge the signatures can give to the interpretation of data when used in combination with the other technologies of modern data science.

% The story we will tell is quite a slow burner, with many core ideas emerging over the last 30 years and now loosely summarised as ``the theory of rough paths''. However, the roots go further back. Core to rough path theory is the mathematical challenge of modelling evolving systems as they interact. The main tool we use to model continuous interactions is calculus. Already for Newton, his calculus provided the controlled differential equations that could be used to explain the interactions between planets. 


==> sections/interpretability.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/interpretability.png}
    \caption{Graphical depiction of the depth 1, 2, and 3 terms of the log-signature for a two-dimensional path $(X^1, X^2)$. \textbf{Left:} The first two depths that includes the change of the variables over the interval and the L\'evy area (shaded). \textbf{Middle and right:} Each plot only varies in a single depth 3 term with other terms being fixed. The middle plot sees varying area density along the $X^2$ axis, and the right along the $X^1$ axis.}
    \label{fig:interpretability}
\end{figure*}

\subsection{Interpretability}
Aside from being grounded in strong mathematical theory, the signature of a path also has geometric meaning. This is of particular interest when learning functions on data, since use of the signature can result in models that are interpretable and explainable. 

The left most plot in Figure \ref{fig:interpretability} contains the visualisations of both the depth 1 and 2 terms of the log-signature. The depth 1 terms are simply the change of the features over the interval; this can be seen directly via
\begin{equation*}
    \logsig^1_{s,t}(\boldsymbol{X}) = \int_{s < u < t} \dd \boldsymbol{X}_u = \boldsymbol{X}_t - \boldsymbol{X}_s = \Delta \mb{X}_{[s, t)}.
\end{equation*}

The depth 2 term is the signed area between the path and the chord joining the endpoints. This is also known as the \textit{L\'evy area} of the path; further examples can be found in \citet{chevyrev2016primer, morrill2020generalised}. 

There exist two more terms at depth 3, however, they are more difficult to visualize directly. However, consider the middle and right plots in \cref{fig:interpretability}. In each plot we draw three curves that differ only in their log-signature values at one of the two depth 3 terms, with the same depth 1 and 2 values.

The plot in the middle shows how one of the terms at depth 3 captures the distribution of the area along the $X^2$ axis. The right most plot demonstrates that the final term captures the extent to which the area has been loaded along the $X^{1}$ axis. 

\begin{example}[Interpretability of breathing data]
    To demonstrate how these features may be interpretable in the context of real data, consider a situation where we are seeking to predict stress from a persons respiratory data (a  problem where signatures have proved very successful). Consider each of the curves in \cref{fig:interpretability} to represent a single breath, with $X^1$ being time and $X^2$ the $\%$ expansion of a band located around the wearers chest that oscillates with breathing \citep[see][]{WESAD2018}.
    
    The values in the signature to depth 1 represent the total time of the breath ($\Delta X^1)$ and the difference in chest expansion from the start and end of the breath ($\Delta X^2$). The depth 2 term (the shaded area) approximates the volume of the inhalation. Finally, the depth 3 term can be seen to represent the sharpness of the inhale (\ref{fig:interpretability}, middle) and the extent to which the breath was a sharp inhale followed by a long exhale, or vice versa.
    (\ref{fig:interpretability}, right).
\end{example}

%% This example serves to demonstrate that the signature terms can be both highly interpretable, as well as highly extensible

Now that we have presented the main mathematical tools in the applications of rough path theory, we describe how these objects are applied in machine learning.



